PID-Comm: A Fast and Flexible Collective Communication Framework for Commodity Processing-in-DIMM Devices

Recent dual in-line memory modules (DIMMs) are starting to support processing-in-memory (PIM) by associating their memory banks with processing elements (PEs), allowing applications to overcome the data movement bottleneck by offloading memory-intensive operations to the PEs. Many highly parallel applications have been shown to benefit from these PIM-enabled DIMMs, but further speedup is often limited by the huge overhead of inter-PE communication. This mainly comes from the slow CPU-mediated inter-PE communication methods which incurs significant performance overheads, making it difficult for PIM-enabled DIMMs to accelerate a wider range of applications. Prior studies have tried to alleviate the communication bottleneck, but they lack enough flexibility and performance to be used for a wide range of applications. In this paper, we present PID-Comm, a fast and flexible collective inter-PE communication framework for commodity PIM-enabled DIMMs. The key idea of PID-Comm is to abstract the PEs as a multi-dimensional hypercube and allow multiple instances of collective inter-PE communication between the PEs belonging to certain dimensions of the hypercube. Leveraging this abstraction, PID-Comm first defines eight collective inter-PE communication patterns that allow applications to easily express their complex communication patterns. Then, PID-Comm provides high-performance implementations of the collective inter-PE communication patterns optimized for the DIMMs. Our evaluation using 16 UPMEM DIMMs and representative parallel algorithms shows that PID-Comm greatly improves the performance by up to 4.20x compared to the existing inter-PE communication implementations. The implementation of PID-Comm is available at https://github.com/AIS-SNU/PID-Comm.

==> AE.tex <==
% LaTeX template for Artifact Evaluation V20201122
%
% Prepared by Grigori Fursin with contributions from Bruce Childers,
%   Michael Heroux, Michela Taufer and other colleagues.
%
% See examples of this Artifact Appendix in
%  * SC'17 paper: https://dl.acm.org/citation.cfm?id=3126948
%  * CGO'17 paper: https://www.cl.cam.ac.uk/~sa614/papers/Software-Prefetching-CGO2017.pdf
%  * ACM ReQuEST-ASPLOS'18 paper: https://dl.acm.org/citation.cfm?doid=3229762.3229763
%
% (C)opyright 2014-2023
%
% CC BY 4.0 license
%

%\documentclass{sigplanconf}

%\usepackage{hyperref}

\cleardoublepage


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% When adding this appendix to your paper, 
% please remove above part
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\appendix
\section{Artifact Appendix}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}

This artifact provides a guide on utilizing the PID-Comm framework, presented in the paper "PID-Comm: A Fast and Flexible Collective Communication Framework for Commodity Processing-in-DIMMs".
We provide the source codes of PID-Comm, along with a short demonstration of how the framework should be used.
For the most recent version of PID-Comm, please refer to the up-to-date artifact link.


\subsection{Artifact check-list (meta-information)}


\begin{itemize}
  \item {\textbf{Run-time environment:} 
  Ubuntu 18.04.}
  \item {\textbf{Hardware:} Multicore x86\_64 CPU with support for AVX512, DDR4 channels equipped with UPMEM DIMMs.}
  \item {\textbf{Metrics:} Functionality check.}
  \item {\textbf{How much disk space required (approximately)?:} 500MB.}
  \item {\textbf{How much time is needed to prepare workflow (approximately)?:} 1 hour.}
  \item {\textbf{How much time is needed to complete experiments (approximately)?:} several minutes.}
  \item {\textbf{Publicly available?:} Yes}
  \item {\textbf{Archived (provide DOI)?:} \url{https://doi.org/10.5281/zenodo.10896568}}
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{How to access}

 Please access the artifact through the provided DOI or through our GitHub link.

\subsubsection{Hardware dependencies}
To use our PID-Comm framework, the following hardware is required.

\begin{itemize}
    \setlength{\itemindent}{0.3cm}
    \item {Multicore x86\_64 CPU with support for AVX512}
    \item {DDR4 channels equipped with UPMEM DIMMs.}
\end{itemize}

Our experiments were tested with a dual-socket Intel Xeon Gold 5215 CPU and 4 DDR4 channels equipped with UPMEM DIMMs.

\subsubsection{Software dependencies}

The following software is required to use the PID-Comm framework.
\begin{itemize}
    \setlength{\itemindent}{0.3cm}
    \item {g++}
    \item {python3.6}
    \item {matplotlib}
    \item {numpy}
    \item {Pandas}
    \item {Scipy}
    \item {UPMEM SDK driver (version 2021.3.0)}
\end{itemize}


\subsubsection{Data sets}

Random-generated datasets were used to demonstrate PID-Comm's primitives.
Other custom datasets may also be used.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Installation}

Install the UPMEM SDK driver (version 2021.3.0), available at \url{https://sdk.upmem.com/}.
After installation, set the UPMEM\_HOME directory to the current library directory, using the upmem\_env.sh script file under the UPMEM-2021.3.0 folder.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}

Of the 8 primitives PID-Comm presents, we take AllReduce as an example and demonstrate its use on a 16-rank UPMEM PIM system (1024 PEs). 
Using the AllReduce\_demo.sh script provided in tutorial/, users can build and execute the tutorial code in the same directory.
The tutorial code will allocate PEs, load data, perform AllReduce between the allocated PEs, and retrieve the final results.
A functionality check is done automatically at the end of each execution.
Users may try out various PE configurations by modifying the given tutorial code.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected results}

PID-Comm will execute desired collective communications between the PEs.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Notes}

Due to the internal architecture of UPMEM DIMMs, there are a few constraints to keep in mind when using PID-Comm. 
Constraints are as follows.
\begin{itemize}
    \setlength{\itemindent}{0.3cm}
    \item {Ranks in use should not include faulty PEs.}
    \item {Each communication group should be larger than 8 PEs.}
    \item {The total size of data in communication should be a multiple of the size of each communication group \texttimes{} 8 bytes.}
\end{itemize}
Be aware that disregarding these constraints will not trigger an error but result in an incorrect output.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% When adding this appendix to your paper, 
% please remove below part
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> backups/apps.tex <==

\section{Benchmark Applications}
\label{sec:apps}
\input{tables/applications_isca}
\NS{add citation for loc-gowalla and livejournal}
To demonstrate how \thiswork can be used to implement important parallel applications and how the proposed library provides speedup, we implement five applications: Deep learning recommendation model (DLRM), graph neural networks (GNN), breadth-first search (BFS), connected components (CC), and multi-layer perceptron (MLP). 
We describe the parallelization strategy and the usage of \thiswork communication model.
Its additional information is depicted in \cref{tab:baselines}.
For those with reference PIM implementations available (GNN, BFS, MLP), we further optimized the baselines to not take unfair advantages.
For those we wrote from scratch (DLRM, CC), we faithfully optimized the kernels and validated all results with CPU implementations.




\subsection{Deep Learning Recommendation Model}
Deep Learning Recommendation Model~\cite{dlrm} (DLRM) is widely used to recommend products or advertisements, based on user information. 
%Its core part is embedding table lookup, where each input is a set of elements which denote the table index to read the vectors from.
It includes lookups to a large embedding table, followed by two linear layers for the final output.
%Also, DLRM utilizes two MLPs to help with recommendations.
%The bottom MLP's output vector and embedding vectors are concatenated and used for feature interaction to create input for the top MLP.
%Finally, we can obtain the results from the top MLP's output.

\subsubsection{Communication Structure}
We follow \cite{dlrmisca} for the 3D parallelization as shown in \cref{fig:dlrm}.
The DLRM architecture is split into tables, rows, and columns, which we map into the hypercube along the $x$, $y$, and $z$ dimensions.
\cref{fig:dlrm} shows the mapping, where we show the communication between four chosen PEs A, C, F, and H.
%which suggests table parallelism, row parallelism, and column parallelism.
%For general implementations, we apply three distinct parallelism concepts along different axes.
%Specifically, we employ table-wise parallelism along the x-axis, row-wise parallelism along the y-axis, and column-wise parallelism along the z-axis.
%This approach involves the use of ReduceScatter once and AlltoAll twice.

%\JU{{\textit{It may be better to use the PID-Comm format. e.g., pidcomm\_alltoall\_xyz, pidcomm\_reducescatter\_y, pidcomm\_alltoall\_xz}}}

The input batch is split according to the divided embedding tables using an AlltoAll in the xyz-space (all PEs).
%Following the embedding lookup, we need to add all embedding vectors from the same table and column to create a complete embedding vector.
Then the complete embedding vector is obtained by performing a ReduceScatter along the y-axis due to the row-wise parallelism.
Finally, the AlltoAll for xz-plane is performed to locate embedding vectors in the correct IDPs for feature interaction and the remaining linear layers.
Scatter and Gather are used at the beginning and the end of the application.
%DLRM underscores the significance of the multi-axis concept because it requires 3D configuration and multiple communications along different axes for performance.

%In the second version, all three parallelisms (3P) are used as an example for using 3-D hypercube.


\subsubsection{Details}
We wrote the DLRM embedding lookup from scratch and validated the output from the reference implementation~\cite{dlrm}.
%Similar to the GNNs, 
We further partitioned the embedding tables given to each PE bank to make sure all data fits into the scratchpad memory and there are enough tasklets to occupy the processor pipeline.
We use Criteo dataset~\cite{criteo}, with two embedding dimensions of 16 and 32.


\subsection{Graph Neural Networks}
Graph Neural Network (GNN) is a relatively new type of deep neural network that takes a graph as the input. %, instead of images or text.
%With some variants, a
A simple GNN layer is composed of two phases: \emph{aggregation} and {combination}. 
%From a vertex, the aggregation collects features from the neighbor vertices, and combination applies a linear learnable layer to the aggregated features.
In a linear algebraic view, they are interpreted as a sparse-dense matrix multiplication (SpGEMM) followed by a dense-dense multiplication (GeMM).

\subsubsection{Communication Structure}
While there can be numerous ways to partition them, we devise two 2D strategies as reasonable examples, similar to existing work~\cite{cagnet, snf}.
We assume each matrix in every layer has to be partitioned, and there is no duplicated multiplication.
In such settings, multi-dimension collective communications are required in each phase. 

In this work, we utilize two configurations, one with ReduceScatter followed by  AllReduce (RS\&AR) and the other with AllReduce followed by AllGather (AR\&AG).
In the (AR\&RS) version shown in \cref{fig:gnn}, the PEs process a 2D tile of the graph topology and a horizontal strip of tiles in the features. 
After aggregation, each PE has a partial sum results of horizontal strips. 
They are ReduceScatter'ed and multiplied to weights for combination.
This will again result in partial sums, which are AllReduce'ed to process aggregation of next layer.
The communication directions will become opposite in every layer.
In the first layer, the data are sent to the PEs via Scatter.
In the last layer the partial sums are Reduce'd to the host to avoid unnecessary AllReduce.

In the AR\&AG strategy, we apply AllReduce instead after aggregation, whose combination leads to 2D tiled results. AllGather will prepare the features in horizontal strips for the next layer.
Note that this one requires Gather instead of Reduce at the last layer.

 

  %  Note that there can be infinitely many configurations on how to split and what communication patterns are used, and what lengths are used for each dimension.
%Because these decisions highly depend on the application characteristics, we focus on the two configuration above to observe the impact of the collective communications.


    
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figs/dlrm_1121_06.pdf}
    \caption{DLRM Communication Structure.}
    \label{fig:dlrm}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth,trim={0 0 0 0},clip]{figs/gnn.pdf}
    \caption{GNN (RS\&AR) Communication Structure. \JL{change to graph}}
    \label{fig:gnn}
\end{figure}



\subsubsection{Details}
After the partitioning, the job of each IDP becomes the local SpGEMM and GEMM.
We faithfully optimized both kernels.
For SpGEMM, we started from the state-of-the-art SpMV implementation SparseP~\cite{sparsep}. 
%Because its input feature is a vector, it suffers from low performance on larger feature width. 
We additionally partitioned the feature matrix into tall matrices to fit into the scratchpad memory, and assign them to tasklets.
For GeMM, @@@.
%
We evaluated GNNs with @@ layers and feature dimension of @@.
We use Pubmed~\cite{pubmed} and Reddit~\cite{reddit} datasets.

\subsection{Breadth First Search}
Breadth-first search (BFS) is an important kernel in graph processing, used to search for the shortest path to a desired node in a given graph. In each iteration, the list of visited nodes is gone through, and the neighbors of visited nodes are marked as visited until there are no unvisited neighbors. We used the reference implementation~\cite{prim} with some optimizations as our baseline. % implementation.

\subsubsection{Communication Structure}
In the baseline implementation, each PE  keeps its own list of visited nodes, and the list is updated at the end of each iteration. Accordingly, AllReduce is used in each iteration for updating the visited list with $or$ reduction. 
%Because the whole list of visited nodes is updated every iteration, BFS spends much time in communication.
\subsubsection{Details}
The reference implementation suffers from inefficient communication and reduction due to serial data transfers and single-threaded reduction operations. We optimized these aspects by changing serial data transfers to parallel, and multi-threading reduction operations, for both the baseline and proposed scheme.
We used Livejournal~\cite{livejournal} and loc-gowalla~\cite{gowalla} for the graph datasets.


\subsection{Connected Component}
Connected Component (CC) is another graph processing application used to search for the number of components in a given graph. 
Each node starts from its own unique label, compares it with the neighboring vertices, and takes the label with a lower value.
%Having the same label means that they are connected.

%For an unvisited node, breadth-first search is performed, marking all connected nodes as visited. This is repeated until all nodes of the graph are visited. We utilized the BFS implementation described above in our baseline implementation. 
\subsubsection{Communication Structure}
CC utilizes a similar communication structure from BFS, which uses AllReduce for each iteration with $min$ reduction. 
In a sense, CC can be viewed as multiple instances of BFS, such that no vertex is left unexplored.
%As CC implementation utilizes BFS from above, they share similar communication structures. 
\subsubsection{Details}
We used the same Livejournal and loc-gowalla datasets. 
We preprocessed directed edges to undirected edges for the graphs for CC to make sense. 

\subsection{Multi-layer Perceptron}
Multi-layer Perceptron (MLP) is a feedforward artificial neural network, frequently used in machine learning. 
Our application performs MLP inference, where each layer carries out GEMM between input weights and feature matrices. We used the reference implementation~\cite{prim} with minor optimizations and changes in communication structure as our baseline implementation
\subsubsection{Communication Structure}
We partition the feature matrix column-wise so that each PE bank receives columns of the feature matrix. Consequently, after a layer is computed, each partial result from PEs is ReduceScatter'ed to each PE before proceeding to the next layer. 
\subsubsection{Microkernel Optimization}
Following \cite{prim}, we used @@\texttimes@@ and @@\texttimes@@ weight parameters.
The model has @@ layers, and ReLU is used as activation at the end of each layer.


==> backups/commmodel_bak_1118.tex <==

\section{\thiswork Communication Model}
\label{sec:model}
In this section, we describe our design for the proposed communication model.
As described in \cref{sec:moti:multi}, there is a need for a model that supports multi-axis collective communication.
On this, we need to achieve two goals, perhaps contradicting each other.
First, the model should provide enough flexibility for users to implement various applications.


, while still achieving high bandwidth (see \cref{sec:moti:mapping}), which might contradict each other.

\SY{Add centralized collective communication here?}
\subsection{Hypercube Communication Topology on PIDs}
\label{sec:model:hypercube}
In this paper, we propose to use a hypercube topology as the communication abstraction.
By letting the users define sizes for a hypercube and map workers onto the hypercube, 
we achieve a good balance between flexibility and performance.

To provide flexibility for multi-axis collective communications, existing libraries for CPUs~\cite{mpitharkur} and GPUs~\cite{nccl} have the notion of \emph{communication group}, which is essentially a user-defined subset of the workers. 
While communication groups can usually be defined as any arbitrary subset, doing so could sabotage the communication bandwidth as exemplified in \cref{sec:moti:entangle}.

One important observation from \cref{sec:moti:entangle} and the DRAM hierarchy is that letting the whole entangled group participate in the communication is crucial for drawing the maximum bandwidth out of the DRAM channel.
That is, either the DPUs forming an entangled group should perform a collective communication among them, or multiple entangled groups should perform communication between each other. 

In such a manner, the hypercube abstraction provides means to force such constraints.
All DPUs are arranged in a hypercube and are physically mapped to the DRAM hierarchy.
\cref{fig:hypercube} (a) shows an example of 4$\times$4$\times$2 hypercube.
For collective communications, the following rules apply.
First, the communication groups are created by selecting one or more dimensions.
For example, only choosing the $X$ dimension as in \cref{fig:hypercube} (b) will create 8 communication groups with size 4.
As another example, choosing the $x$ and $z$ dimensions will create 2 communication groups of size $4\times 4$ as shown in \cref{fig:hypercube} (c).
On the other hand, Figure shown in \cref{fig:hypercube} (d) is illegal because it splits the $x$ dimension. 
Second, when a collective communication API is invoked, all created groups will participate. 
This will ensure that an entire entangled group is always accessed together, and allows the host processor to efficiently process them.
Third, the root of centralized collective communication is always the host processor. 
This is reasonable because using only a single DPU to perform any computation will be inferior to using the host processor to do the same job.
This approach diverges from Chen et al.~\cite{simplepim}, which only allows a single group of IDPs to interact with a singular type of communication.

Please note that the model slightly restricts forming irregular communication groups, such as groups of different sizes, or of overlapping members.
However, most of the applications using collective communications exhibit regular structures that fit the hypercube topology~\cite{zero, fft, megatron, some, more}, and thus the choice incurs very little restriction in practice.
On the other hand, the performance benefit gained from this design choice is significant, as we will demonstrate in the experimental results.




\subsection{Hypercube Formatting}
\label{sec:mapping:format}


We define a canonical format that describes an $D$-dimensional hypercube as a vector with the dimension size in each element.
For example, $[4,2,4]$ indicates a $4\times 2\times 4$ hypercube shown in \cref{fig:hypercube} (a). 
%Note that there can be $D(D-1)$ duplicate descriptions for an identical hypercube because the order of dimensions does not matter.
Using this format, the user must first provide the length of each axis. 
On top of the hypercube description, the user provides a list of collective communications on the desired communications with one-hot vectors to depict communicating dimensions.
For example, the series of communications illustrated in \cref{fig:hypercube} (b) and (c) are described as $[1,0,0, \mathit{RS}]$ followed by $[1,0,1,\mathit{AA}]$. \JU{The library also needs data size}
We do not allow a partial dimension of the hypercube to perform collective communication. 
When such communication is needed, the hypercube should be defined with an extra dimension, which does not restrict the flexibility of the model.
Additionally, the user can provide whether each axes should be mapped to entangled or orthogonal groups using bitmaps. \SY{Does this make sense?} 


\subsection{Hypercube Mapping}
\SY{Will change prime numbers to actual numbers}
In this section, we describe how the user's input affects the mapping between the virtual hypercube and physical banks.
Once the user provides the number of dimensions and the size of each dimension (e.g., $L \times M\times N$), the hypercube is mapped to the physical banks of the PIM-enabled DIMMs.
The physical dimensions of PID banks are organized as $Ch\times R \times C \times B$, whose literals stand for \underline{Ch}annel, \underline{R}ank, \underline{C}hip, and \underline{B}ank (e.g., $4Ch\times 4R \times 8C \times 8B$).

The key aspect of mapping is that we maintain alignment on the entangled groups in the DIMMs. 
While there could be various mapping methods to do so, we map the hypercube dimensions of lower IDs to the entangled group first (`C' dimension), and the rest dimensions will fill the DRAM hierarchy from bottom to top (C-B-R-Ch).
%These physical banks are mapped onto a hypercube of . %, \thiswork maps it to the physical PID based on prime factorization. %, because it is infeasible to map dimensions between different primes factors.
%Prime-factor the dimension sizes and group them based on the primes. 
%In the case depicted in \cref{fig:hypercube}, $2$ is the only prime number: $2^l \times 2^m\times 2^n$ hypercube and $2^{ch}\times 2^r \times 2^c \times 2^b$ PID banks.
%We then map the dimension on the matching position. 
A toy example mapping between $[l=3, m=1, n=2]$ and $[ch=1, r=1, c=2, b=2]$ is illustrated in \cref{fig:mapping}. The $n=2$ dimension occupies 4 chips in the same bank.
Then two such banks form $m=1$ dimension, and 8 of these form the last dimension of $l=3$.

One implication is that while there seems to be no difference between the dimensions of the hypercube, the underlying communication will be drastically different based on how they are mapped. 
In particular, communication of banks within the entangled group and across the entangled groups will exhibit huge differences in its pattern.
\thiswork handles such different communication transparent from the users with high performance. 
Please refer to the next section for the high-performance optimizations and implementation details for the collective communication primitives.





\subsection{Hypercube Formatting}
\label{sec:mapping:format}

\JL{we probably don't need this section any more}


We define a canonical format that describes an $D$-dimensional hypercube as a vector with the dimension size in each element.
For example, $[4,2,4]$ indicates a $4\times 2\times 4$ hypercube shown in \cref{fig:hypercube} (a). 
%Note that there can be $D(D-1)$ duplicate descriptions for an identical hypercube because the order of dimensions does not matter.
Using this format, the user must first provide the length of each axis. 
On top of the hypercube description, the user provides a list of collective communications on the desired communications with one-hot vectors to depict communicating dimensions.
For example, the series of communications illustrated in \cref{fig:hypercube} (b) and (c) are described as $[1,0,0, \mathit{RS}]$ followed by $[1,0,1,\mathit{AA}]$. \JU{The library also needs data size}
We do not allow a partial dimension of the hypercube to perform collective communication. 
When such communication is needed, the hypercube should be defined with an extra dimension, which does not restrict the flexibility of the model.
Additionally, the user can provide whether each axes should be mapped to entangled or orthogonal groups using bitmaps. \SY{Does this make sense?} 


==> backups/motiv_back_1120.tex <==
\section{Motivation} % <-- YS's suggestion
\label{sec:motiv}

% \JL{
% check if these goals are all taken:
% 1. why comm is important
% 2. why commlib is slow (or why it is difficult)
% 3. why comm model is important
% }


\subsection{Conventional Communication Models and Libraries}
\label{sec:moti:conventional}
%%SY copied from the next section
It is well known that commodity PIM-enabled DIMMs suffer from poor inter-PE communication~\cite{prim, pidjoin, pimulator}.
In \cite{prim}, multiple applications are classified into PIM-friendly and PIM-unfriendly, and the unfriendliness is often caused by inter-PE communication. \SY{changed the words to PIM-friendly from PID-friendly.}
The same phenomenon is reported in many literature~\cite{pidjoin, sparsep, upmemtraining}.
Particularly in the context of modern machine learning and scientific applications, where inter-PE communication is crucial, addressing this issue cannot be overlooked.
However, currently, no communication model has been well-established for PIM-enabled DIMMs.
%In the commercial product UPMEM~\cite{upmem}, the programming model is defined as 
Commodity UPMEM PIM-enabled DIMMs define their programming model as a shared-nothing structure~\cite{upmem}, where each PE is meant to run independently until the control gets transferred back to the host CPUs.
For this, the set of currently supported communication APIs in UPMEM SDK is CPU to PEs, such as parallel read, parallel write, and broadcast.
This indicates that any inter-PE communication is left outside the programming model. 
Users are responsible for writing host-side programs for any data movement between and redistribution to the PEs' MRAMs and launching the next kernels.
Some alternative programming models for PIM-enabled DIMMs have been proposed~\cite{nda, bufcmp}, but they adopt similar host-centric approaches.
Additionally, while Chen et al.~\cite{simplepim} does provide a general programming framework for UPMEM and (albeit limited) functions for collective communication, it still does not provide an efficient communication model.  

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/motiv_flow.pdf}
    \caption{Communicaiton flow of prior work and \thiswork.}
    \label{fig:moticomm}
\end{figure}

We identify the lack of a well-defined communication model as an important factor in the high inter-PE communication overheads of the PIM-enabled DIMMs and applications.
%current communication bottleneck for PID-accelerated programs.
Without native hardware support for inter-PE communication (e.g., physical channels),
%available for communication between the banks, 
the only medium for the communication is the host CPU which becomes the sole component in charge of handling all the rearrangement and arithmetic needed for the communication.
For example, \cref{fig:moticomm} shows how AlltoAll can be performed using the conventional inter-IDP communication model of the UPMEM DIMMs.
\SY{Change after figure is completed}
\circled{1} The data are sent to the host's vector registers, and \circled{2} the domain transfer is automatically applied toward the host domain.
\circled{3} The host spills the contents to host memory \circled{4} to perform data rearangement.
Multiple steps of data rearrangement are necessary, involving numerous accesses to host memory. 
This is because data destined for the same PID devices' banks is scattered across memory.
\circled{5} After moving the contents back to the vector register, \circled{6} the domain is transferred back to the PID domain.
\circled{5} Sending these data to the PID devices' banks completes the communication.

\SY{Removed some spoilers, but now seems too short...}
Unfortunately, this model has three significant problems. 
First, data rearrangement (and reduction for collective primitives such as ReduceScatter and AllReduce) is done single-handedly by the host. 
This causes the host CPU to become a significant performance bottleneck. 
Second, spilling data to host memory causes a large overhead. %would have been eliminated if each vector register already held the necessary target data.
%In other words, if the data in the DPU were arranged in a specific manner, the host memory operation could have been done simultaneously within each vector register.
Third, domain transfer is done for all of the data that reaches the host. 
%hogging host resources despite only being necessary when the host performs arithmetic computations. 
%Given that the host is solely involved in data rearrangement in the current scenario, we can remove domain transfers without losing functionality.
These three main issues cause the overall communication flow to become highly ineffective. 
On the contrary, \thiswork addresses and solves these challenges through designated techniques, resulting in a more efficient communication flow. 
We analyze the overhead caused by these three problems in conventional inter-PE communication and how we solve it in the next section (\cref{sec:moti:app}).



\begin{comment}
First, it consumes most of the time on the two domain transfers.
As the domain transfer is essentially a global transpose, the host CPUs need to perform multiple SIMD instructions per cache line. 
Even with AVX-512 extension, it has to undergo three instructions per every cacheline.
Second, all the calculations, including the domain transfer, inter-cacheline arrangement, and reduction are performed by the host CPUs. 
This makes the host CPUs become a major performance bottleneck and the PID devices not scalable.
%which is the cause of 
%and thus increasing the number of memory channels has minimal impact on the execution time as seen in \cref{sec:moti:app}.
\end{comment}

\begin{comment}
\begin{figure}[t]
    \centering
    \includegraphics[width=.85\columnwidth]{figs/motilib.pdf}
    \caption{Throughput of conventional collective communication methods. }
    \label{fig:motilib}
\end{figure}

The throughput of the collective communication functions written in such a way is plotted in \cref{fig:motilib}.
It is clear that most of the collective communication primitives severely suffer from low bandwidth, far below that of the theoretical max bandwidth from the external bus (4 channels\x 19.2GB/s).
The only exception is AllGather, which sustains about half of the theoretical peak bandwidth utilization.
This is a strong indicator of the host CPU being the bottleneck.
When the data are AllGathered, most of the communication time is spent on the PID-to-CPU side due to its larger data size than the opposite direction. %sending the large amount of data the host CPU to the PID banks, the same set of data are sent to multiple entangled groups. 
Because of this, the host CPU can reuse the result of domain transfers among multiple IDPs.
However, for all the other three, such a trick cannot be used, and they all suffer from the huge CPU overhead of domain transfer.
%This greatly reduces the processor burden.
In the novel communication library provided as a part of this work, we reduce/offload the burden of the host and achieve multifold speedup on these collective primitives.
\end{comment}


\subsection{Lack of Flexible Communication}
\label{sec:moti:multi}
\SY{WIP}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{scratchfigs/motiv_entangled}
    \caption{Bandwidth comparison of communication within entangled and non-entangeld groups.}
    \label{fig:moticomm}
\end{figure}

There are multiple applications that require diverse forms of collective communications with different source and destination node groups~\cite{dlrm, gnn, fft}. 
For a library to support such applications, two conditions must be satisfied.
First, the library must have building blocks that are general enough to accommodate the different types of collective communications. 
Among existing prior work, Gómez-Luna et al.~\cite{upmemtraining} and Lim et al.~\cite{pidjoin} do not meet this requirement since they focus on a single application. 
Second, the library must have sufficient flexibility to allow participating nodes to communicate with different groups of nodes within a single application runtime.
In other words, the library should group nodes based on their collective communication pattern, and easily reconfigure nodes into new groups to accommodate new patterns.  
Chen et al.~\cite{simplepim} fails to meet this criterion as it only supports a single group of nodes. 
Once a group of nodes is fixed at the start of the application, communication is confined within that specific group configuration throughout the entire application duration. 
In conclusion, there is no inter-IDP communication library that can support applications with diverging communication patterns. 


\subsection{Large Overhead on Inter-IDP Communication}
\label{sec:moti:app}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{scratchfigs/motiv_comm_breakdown_real.png}
    \caption{Execution time breakdown of PID applications. \SY{DLRM is dummy value}}
    \label{fig:motiperf}
\end{figure}


To demonstrate the impact of poor inter-PE communication, we breakdown the execution times of multiple application scenarios on PIM-enabled DIMMs (see \cref{sec:apps} for details).
In each application in \cref{fig:motiperf}, the left bar represents the execution time breakdown into computation and inter-PE communication.
Next, the right bar provides a detailed breakdown of inter-PE communication. 
It is evident that the majority of the execution time is spent on communication.
This trend persists for all applications of several environments and indicates that inter-PE communication is a major performance bottleneck. 
Within inter-PE communication, domain transfer takes the longest, followed by host memory access and data rearrangement\slash reduction.
In the novel communication library introduced in this work, we offload the burden of the host and achieve multifold speedup on collective primitives.



\begin{comment}

\subsection{Impact of IDP Placements on Communication}
\label{sec:moti:mapping}
The existing UPMEM programming model regards all IDPs to be perfectly symmetric.
However, this could cause severe problems for inter-IDP communication.


\subsection{Impact of IDP Placements}
\label{sec:moti:mapping}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{scratchfigs/motibw.pdf}
%     \caption{Read/write bandwidth measured from sets of eight PID banks. \JL{let's merge fig6 and fig7}}
%     \label{fig:motibw}
% \end{figure}

\JL{this might be too trivial?}
As explained in \cref{sec:background}, the PID banks are not totally independent, especially because of the entangled groups.
For communications, this architecture plays a crucial role in achieving high performance.

%In \cref{fig:moti:mapping}, we have plotted the bandwidth of reading/writing data from eight PID banks.

We have selected a set of eight random banks, eight banks from the same chip, eight banks from the same chip of different channels, and eight banks from the entangled group (i.e., eight chips of the same DIMM, same local bank IDs). 
When a random mapping is considered, the bandwidth is significantly low. 
Interestingly, the bandwidth from banks from the same chip shows even lower bandwidth. 
This is because such a choice allows the use of 1/8 of the total pin count for the transfer. 
On the other hand, reading and writing from an entangled group achieves @@ GBps, close to the peak DDR bandwidth and equal to that of the all 64 banks in a DIMM.
This results emphasize that an appropriate mapping of the programs to banks is important for the inter-bank communication.


    
\end{comment}

==> cover_letter_backups/240220_index_backup.tex <==
\bookmark[level=0]{Revision document}
{

\begin{center}
{\large{\textbf{\textsc{Response to Reviewer Comments}}}}
\end{center}

% \vspace{1mm}


\begin{center}
\setlength{\fboxrule}{1pt}
\fbox{\begin{minipage}{0.95\columnwidth}We sincerely thank the reviewers for their time and valued comments. We have faithfully revised our paper and addressed each reviewer's comments below with much appreciation. All the revised texts are written in {\color{olivegreen}green color} with magenta markers {\color{magenta}{R$i$D$k$, MR1-MR6}} around them. Please refer to the overall requests below with \underline{hyperlinks} to them. Note that the term `Reviewer $i$D$k$' means the discussion point $k$ from the reviewer $i$.
\end{minipage}} 
\end{center}

% %%% Meta Reviewer Section %%%
     
% \setcounter{section}{1}
% \section*{For the Meta-Reviewer (Overall Requests)}
% \phantomsection
% \bookmark[dest=meta_reviewer, level=1]{Meta Reviewer}

% {
% \hypertarget{meta_reviewer}{}



% %%% Meta Reviewer 1.1 subsection %%%
% \subsection{Discuss and evaluate the overhead in memory consumption. [Reviewer 5D1]}
% {
% %%% Meta Reviewer 1.1 subsection %%%

% Thank you for the request on memory usage analysis.
% In \figref{memory_analysis} and \revref{MR1} (p.10, left), we analyzed how efficient \thiswork is on memory usage and how expansion-aware sampling mitigates the neighbor explosion in deep GNNs (\figref{memory_analysis}a).
% Additionally, we showed that \thiswork can handle large graphs which the full-graph training cannot by transitioning to mini-batch training using \cobatch. \thiswork tries to use limited memory as efficiently as possible, especially when the graph is too large to be handled by the full-graph training (\figref{memory_analysis}b).

% }


% }

%%% Reviewer 1 Section %%%

% \vspace{3mm}
\setcounter{section}{1}
\section*{For Reviewer \#1}
\phantomsection
\bookmark[dest=reviewer1, level=1]{Reviewer \#1}
\setcounter{subsection}{0}

{
\hypertarget{reviewer1}{}

\subsection{D1: Justification of Using PIM-Enabled DIMMs}
\SY{Written on the assumption that only BFS \& CC are slower}
Thank you for the suggestion. 
We have added CPU baselines to \figref{eval:benchmark} for a better demonstration of the high-performing PIM-enabled DIMMs.
While most benchmark applications benefit from PIM-enabled DIMMs, BFS and CC are slower due to the large inter-PE communication portion in the execution time. 
Despite this, \thiswork achieves @@ speedup compared to the PIM-enabled DIMM baseline.

\subsection{D2: Using PEs to Accelerate Computation}
We apologize for the confusion. 
In \figref{eval:benchmark}, for PIM-enabled DIMM baseline and \thiswork, `Compute' represents the portion of execution time on computation on PEs. 
\SY{Is the following necessary?}
To avoid additional confusion, we use different color-coding for computation on the CPU and PIM-enabled DIMMs in \figref{eval:benchmark}.

\subsection{D2: \thiswork with Multi-Host Environment}
Experimental results - Utilize dual-socket for multi-host environment experiment.

}


%%% Reviewer 2 Section %%%

% \vspace{3mm}
\setcounter{section}{2}
\section*{For Reviewer \#2}
\phantomsection
\bookmark[dest=reviewer2, level=1]{Reviewer \#2}
\setcounter{subsection}{0}

{
\hypertarget{reviewer2}{}

\subsection{D1: \thiswork with Other PIM Architectures}
Section~\ref{sec:discussion:otherpimarch} and Figure~\ref{fig:discussion:otherpimarch} are newly added on page~12.
This section explores the applicability of \thiswork{} for other PIM architectures. 
They show how \thiswork{} is implemented on two alternative real-world PIM architectures: Samsung HBM-PIM~\cite{hbmpim} and Samsung AxDIMM~\cite{axdimm}. 
It is demonstrated that, notwithstanding the diverse characteristics of these PIM architectures, \thiswork{} consistently exhibits significant bandwidth improvements for \hl{all} categories of collective communication primitives on those architectures.



\subsection{D2: Replacing Vector Instructions with Intel DSA}
Experimental results - to compare data modulation performance of AVX512 with intel DSA, 

\subsection{D3: Implementing Collective Communications with CXL NMP}
Discussion - yes the same techniques will work in CXL NMPs too. detailed explanation to add later

\subsection{D4: Separating Performance Benefits between PIM-Enabled DIMMs and \thiswork}

\SY{Same with R1D1} 
divide into PIM-friendly and PIM-unfriendly, show most applications in the benchmark are
Faster than CPU baseline (reference to figure), explanation on BFS and CC

}

%%% Reviewer 3 Section %%%

% \vspace{3mm}
\setcounter{section}{3}
\section*{For Reviewer \#3}
\phantomsection
\bookmark[dest=reviewer3, level=1]{Reviewer \#3}
\setcounter{subsection}{0}

{
\hypertarget{reviewer3}{}

\subsection{D1: Figures' Font size}
We apologize.
We increased the font size of figures in {\color{olivegreen}green boxes} labeled as @@.

\subsection{D2: Non-PIM Baseline}
\SY{Same with R1D1}
divide into PIM-friendly and PIM-unfriendly, show most applications in the benchmark are
Faster than CPU baseline (reference to figure), explanation on BFS and CC

\subsection{D3: Optimization compared to SimplePIM~\cite{simplepim}}
%Discussion - Simplepim's implementations are unoptimized in that the three schemes (avoid transpose, evade hostmem, pim-assisted reordering) in the paper are not applied. We applied the 3 schemes in the library implementations. Primitives already implemented in SimplePIM also benefit performance-wise in our new implementation. (See figure 14, base is SimplePIM)
We apologize for the confusion. 
The main difference of \thiswork compared to SimplePIM is three-fold: using optimization techniques for collective communication operations as shown in \tblref{techniques},  allowing multi-dimensional collective communication with virtual hypercube model, and supporting additional primitives (AA, RS, Re) as in \tblref{prior}.  
Performance comparison between SimplePIM and \thiswork can be located in \figref{eval:centprim}.

}

%%% Reviewer 4 Section %%%

% \vspace{3mm}
\setcounter{section}{4}
\section*{For Reviewer \#4}
\phantomsection
\bookmark[dest=reviewer4, level=1]{Reviewer \#4}
\setcounter{subsection}{0}

{
\hypertarget{reviewer4}{}

\subsection{D1: Comparison with Hierarchy-Aware Approaches}

Thank you for your comment on the potential effects of other hierarchy-aware approaches.
Section~\ref{} and Figure~\ref{} are newly added on page~X.
This section shows the effects of the hierarchy-aware approach based on the DIMMs' memory architecture.
It is shown that performing collective communication concerning the DIMM's memory hierarchy (e.g., banks, chips, and ranks) has a negligible impact on the bandwidth of \thiswork. 

\subsection{D2: Clarifying Baseline Measurement}

We apologize for the confusion and appreciate the advice on improving the clarity of the baseline system configuration setups.
Both SimplePIM~\cite{simplepim} and \thiswork were evaluated for performance on an UPMEM-enabled system.
Additionally, to fix the misleading description of the CPIstack method in \secref{eval:benchmark}, we revised the following sections:

\begin{itemize}
    \item \secref{eval:setup}: We explicitly state that all baselines and \thiswork is implemented and measured on a real system. 
    \item \secref{eval:benchmark}: For \figref{eval:benchmark}, we have not used any CPIstack-related methods for breakdown and instead measured the execution time of each portion on a real system. Thus, we remove this description. 
    \item \secref{eval:ablation}: For \figref{eval:Primitive_breakdown}, we have used a CPIstack-like method on a real system to break down sections that highly overlap. We added the related description and reference accordingly. 
\end{itemize}

\subsection{D3: Applying \thiswork to Different Communication Networks on PIM-Enabled DIMMs and future generation PIM}
discussion. 
comm. still needed. ex)HBM PIM

}

%%% Reviewer 5 Section %%%

% \vspace{3mm}
\setcounter{section}{5}
\section*{For Reviewer \#5}
\phantomsection
\bookmark[dest=reviewer5, level=1]{Reviewer \#5}
\setcounter{subsection}{0}

{
\hypertarget{reviewer5}{}

\subsection{D1: Gather/Broadcast Latencies in the Benchmarks}

Clarify \& modify figure 
% 
%% ?? 

\subsection{D2: PE-Assisted Reordering Overhead}
% Clarify - reordering overhead is already included in each primitive execution time.
The overhead of PE-assisted reordering is already accounted for in the execution time.
Figure~\ref{} shows a breakdown of the execution time of four communication primitives.
The specific category labeled "PE-side modulation" in the breakdown represents the overhead introduced by PE-assisted reordering.
We add further discussion on this overhead in Section~\ref{}.

\subsection{D3: Bandwidth Requirements of Broadcast}
%% Clarify - fig 14's results are performance measurements of primitives on our system setup. It doesn't necessarily mean that broadcast requires very high bandwidth, but rather that it shows the highest performance compared to other primitives in the same setup.


\subsection{D4: PE-Assisted Reordering in Reduce Scatter}
%% Clarify - Reordering enables storing data with different destinations in one vector register. After in-register rotation is performed, data with the same destination is located in the same index of the vector register. Finally, inter-vector register addition is performed for results.

}

}




==> cover_letter_backups/240221_1_index_backup_somewhat_filled.tex <==
\bookmark[level=0]{Revision document}
{

\begin{center}
{\large{\textbf{\textsc{Response to Reviewer Comments}}}}
\end{center}

% \vspace{1mm}


\begin{center}
\setlength{\fboxrule}{1pt}
\fbox{\begin{minipage}{0.95\columnwidth}We sincerely thank the reviewers for their time and valued comments. We have faithfully revised our paper and addressed each reviewer's comments below with much appreciation. All the revised texts are written in {\color{olivegreen}green color} with magenta markers {\color{magenta}{R$i$D$k$, MR1-MR6}} around them. Please refer to the overall requests below with \underline{hyperlinks} to them. Note that the term `Reviewer $i$D$k$' means the discussion point $k$ from the reviewer $i$.
\end{minipage}} 
\end{center}

% %%% Meta Reviewer Section %%%
     
% \setcounter{section}{1}
% \section*{For the Meta-Reviewer (Overall Requests)}
% \phantomsection
% \bookmark[dest=meta_reviewer, level=1]{Meta Reviewer}

% {
% \hypertarget{meta_reviewer}{}



% %%% Meta Reviewer 1.1 subsection %%%
% \subsection{Discuss and evaluate the overhead in memory consumption. [Reviewer 5D1]}
% {
% %%% Meta Reviewer 1.1 subsection %%%

% Thank you for the request on memory usage analysis.
% In \figref{memory_analysis} and \revref{MR1} (p.10, left), we analyzed how efficient \thiswork is on memory usage and how expansion-aware sampling mitigates the neighbor explosion in deep GNNs (\figref{memory_analysis}a).
% Additionally, we showed that \thiswork can handle large graphs which the full-graph training cannot by transitioning to mini-batch training using \cobatch. \thiswork tries to use limited memory as efficiently as possible, especially when the graph is too large to be handled by the full-graph training (\figref{memory_analysis}b).

% }


% }

%%% Reviewer 1 Section %%%

% \vspace{3mm}
\setcounter{section}{1}
\section*{For Reviewer \#1}
\phantomsection
\bookmark[dest=reviewer1, level=1]{Reviewer \#1}
\setcounter{subsection}{0}

{
\hypertarget{reviewer1}{}

\subsection{D1: Justification of Using PIM-Enabled DIMMs}
Thank you for the suggestion. 
We have added CPU baselines to \figref{@@} for a better demonstration of the high-performing PIM-enabled DIMMs.
The PIM baseline reflects the difficulty of fully utilizing PIM-enabled DIMM to outperform the CPU baseline due to its slow communication, especially for communication-heavy baselines such as @@ and @@. 
Despite this, \thiswork achieves @@ speedup compared to the PIM-enabled DIMM baseline due to effective communication.

\subsection{D2: Using PEs to Accelerate Computation}
We apologize for the confusion. 
In \figref{eval:benchmark}, for PIM-enabled DIMM baseline and \thiswork, `Compute' represents the portion of execution time on computation on PEs. 
\SY{Is the following necessary?}
To avoid additional confusion, we use different color-coding for computation on the CPU and PIM-enabled DIMMs in \figref{eval:benchmark}.

\subsection{D2: \thiswork with Multi-Host Environment}
% Experimental results - Utilize dual-socket for multi-host environment experiment.
Thank you for the suggestion. 
\thiswork can be applied to multi-host environments by adding another step of communication between multiple hosts. 
Other than this additional step, the designs of \thiswork can be fully utilized. 
To demonstrate this, we added a new experimental result in \ref{} by emulating the multi-host environment using two processes allocated to different sockets. 
Additionally, we share the expected performance of a multi-host environment with different communication standards. 
}


%%% Reviewer 2 Section %%%

% \vspace{3mm}
\setcounter{section}{2}
\section*{For Reviewer \#2}
\phantomsection
\bookmark[dest=reviewer2, level=1]{Reviewer \#2}
\setcounter{subsection}{0}

{
\hypertarget{reviewer2}{}

\subsection{D1: \thiswork with Other PIM Architectures}
Section~\ref{sec:discussion:otherpimarch} and Figure~\ref{fig:discussion:otherpimarch} are newly added on page~12.
This section explores the applicability of \thiswork{} for other PIM architectures. 
We explain in detail that as long as certain communication paths rely on the host, \thiswork's motivation and design can still give insight, albeit implementation details differ. 
\begin{comment}
They show how \thiswork{} is implemented on two alternative real-world PIM architectures: Samsung HBM-PIM~\cite{hbmpim} and Samsung AxDIMM~\cite{axdimm}. 
It is demonstrated that, notwithstanding the diverse characteristics of these PIM architectures, \thiswork{} consistently exhibits significant bandwidth improvements for \hl{all} categories of collective communication primitives on those architectures.
\end{comment}


\subsection{D2: Replacing Vector Instructions with Intel DSA}
%Experimental results - to compare data modulation performance of AVX512 with intel DSA, 
Thank you for the suggestion. 
While Intel DSA is a useful tool for alleviating the memory management burden of the host, the current DSA does not include the necessary functions for data modulation, such as shifting. 
However, once these requirements are met, we expect that this could accelerate data modulation even more. 

\subsection{D3: Implementing Collective Communications with CXL NMP}
% Discussion - yes the same techniques will work in CXL NMPs too. detailed explanation to add later
\SY{Same with R2D1}


\subsection{D4: Separating Performance Benefits between PIM-Enabled DIMMs and \thiswork}
\SY{Same with R1D1} 
%divide into PIM-friendly and PIM-unfriendly, show most applications in the benchmark are Faster than CPU baseline (reference to figure), explanation on BFS and CC

}

%%% Reviewer 3 Section %%%

% \vspace{3mm}
\setcounter{section}{3}
\section*{For Reviewer \#3}
\phantomsection
\bookmark[dest=reviewer3, level=1]{Reviewer \#3}
\setcounter{subsection}{0}

{
\hypertarget{reviewer3}{}

\subsection{D1: Figures' Font size}
We apologize.
We increased the font size of figures in {\color{olivegreen}green boxes} labeled as @@.

\subsection{D2: Non-PIM Baseline}
\SY{Same with R1D1}
%divide into PIM-friendly and PIM-unfriendly, show most applications in the benchmark are Faster than CPU baseline (reference to figure), explanation on BFS and CC

\subsection{D3: Optimization compared to SimplePIM~\cite{simplepim}}
%Discussion - Simplepim's implementations are unoptimized in that the three schemes (avoid transpose, evade hostmem, pim-assisted reordering) in the paper are not applied. We applied the 3 schemes in the library implementations. Primitives already implemented in SimplePIM also benefit performance-wise in our new implementation. (See figure 14, base is SimplePIM)
We apologize for the confusion. 
The main difference of \thiswork compared to SimplePIM is three-fold: using optimization techniques for collective communication operations as shown in \tblref{techniques},  allowing multi-dimensional collective communication with virtual hypercube model, and supporting additional primitives (AA, RS, Re) as in \tblref{prior}.  
Performance comparison between SimplePIM and \thiswork can be located in \figref{eval:centprim}.

}

%%% Reviewer 4 Section %%%

% \vspace{3mm}
\setcounter{section}{4}
\section*{For Reviewer \#4}
\phantomsection
\bookmark[dest=reviewer4, level=1]{Reviewer \#4}
\setcounter{subsection}{0}

{
\hypertarget{reviewer4}{}

\subsection{D1: Comparison with Hierarchy-Aware Approaches}
\begin{comment}
Thank you for your comment on the potential effects of other hierarchy-aware approaches.
Section~\ref{} and Figure~\ref{} are newly added on page~X.
This section shows the effects of the hierarchy-aware approach based on the DIMMs' memory architecture.
It is shown that performing collective communication concerning the DIMM's memory hierarchy (e.g., banks, chips, and ranks) has a negligible impact on the bandwidth of \thiswork. 
\end{comment}
Thank you for the suggestion.
To demonstrate the effectiveness compared to our virtual hypercube, we tested additional topologies (ring, tree) within the PIM-enabled DIMM in @@.
This indicates that compared to other baselines, our virtual hypercube achieved the highest performance due to using the entangled group as the smallest effective unit for flexible communication. 

\subsection{D2: Clarifying Baseline Measurement}

We apologize for the confusion and appreciate the advice on improving the clarity of the baseline system configuration setups.
Both SimplePIM~\cite{simplepim} and \thiswork were evaluated for performance on an UPMEM-enabled system.
Additionally, to fix the misleading description of the CPIstack method in \secref{eval:benchmark}, we revised the following sections:

\begin{itemize}
    \item \secref{eval:setup}: We explicitly state that all baselines and \thiswork is implemented and measured on a real system. 
    \item \secref{eval:benchmark}: For \figref{eval:benchmark}, we have not used any CPIstack-related methods for breakdown and instead measured the execution time of each portion on a real system. Thus, we remove this description. 
    \item \secref{eval:ablation}: For \figref{eval:Primitive_breakdown}, we have used a CPIstack-like method on a real system to break down sections that highly overlap. We added the related description and reference accordingly. 
\end{itemize}

\subsection{D3: Applying \thiswork to Different Communication Networks on PIM-Enabled DIMMs and future generation PIM}
%comm. still needed. ex)HBM PIM
\SY{Same with R2D1}

}

%%% Reviewer 5 Section %%%

% \vspace{3mm}
\setcounter{section}{5}
\section*{For Reviewer \#5}
\phantomsection
\bookmark[dest=reviewer5, level=1]{Reviewer \#5}
\setcounter{subsection}{0}

{
\hypertarget{reviewer5}{}

\subsection{D1: Gather/Broadcast Latencies in the Benchmarks}

% Clarify \& modify figure 
\SY{Is this the best answer?}
We apologize for the confusion. 
As shown in \tblref{baselines}, DLRM and GNN AR\&AG include the gather primitive, and DLRM, BFS and CC include the broadcast primitive, albeit a relatively small portion. 
We have increased the height of \figref{eval:benchmark} to provide a clearer view of the two primitives. 

\subsection{D2: PE-Assisted Reordering Overhead}
% Clarify - reordering overhead is already included in each primitive execution time.
The overhead of PE-assisted reordering is already accounted for in the execution time.
Figure~\ref{} shows a breakdown of the execution time of four communication primitives.
The specific category labeled "PE-side modulation" in the breakdown represents the overhead introduced by PE-assisted reordering.
We add further discussion on this overhead in Section~\ref{}.

\subsection{D3: Bandwidth Requirements of Broadcast}
%% Clarify - fig 14's results are performance measurements of primitives on our system setup. It doesn't necessarily mean that broadcast requires very high bandwidth, but rather that it shows the highest performance compared to other primitives in the same setup.
We apologize for the confusion. 
\figref{eval:centprim} compares the performance by measuring the bandwidth of each primitive. 
The y-axis does not imply bandwidth requirements but the performance of the primitive (higher, the better).
Thus, in the figure broadcast shows high performance for both baseline and \thiswork. 


\subsection{D4: PE-Assisted Reordering in Reduce Scatter}
%% Clarify - Reordering enables storing data with different destinations in one vector register. After in-register rotation is performed, data with the same destination is located in the same index of the vector register. Finally, inter-vector register addition is performed for results.
We apologize for the confusion. 
To utilize AVX's vector sum operations, values to be added must reside in different registers. 
Thus, if PE-assisted reordering were not used, the host would have to redistribute the data within the host memory and then read the redistributed data back to separate vector registers, causing additional memory access overhead. 
This applies to both ReduceScatter and AllReduce.
\SY{Modify main paper as well?}
}

}




==> cover_letter_backups/240221_2_index_backup_split_reviewer.tex <==
\bookmark[level=0]{Revision document}
{

\begin{center}
{\large{\textbf{\textsc{Response to Reviewer Comments}}}}
\end{center}

% \vspace{1mm}


\begin{center}
\setlength{\fboxrule}{1pt}
\fbox{\begin{minipage}{0.95\columnwidth}We sincerely thank the reviewers for their time and valued comments, and apologize for any confusion. We have faithfully revised our paper and addressed each reviewer's comments below with much appreciation. All the revised texts are written in {\color{olivegreen}green color} with magenta markers {\color{magenta}{R$i$D$k$, MR1-MR6}} around them. Please refer to the overall requests below with \underline{hyperlinks} to them. Note that the term `Reviewer $i$D$k$' means the discussion point $k$ from the reviewer $i$.
\end{minipage}} 
\end{center}

% %%% Meta Reviewer Section %%%
     
% \setcounter{section}{1}
% \section*{For the Meta-Reviewer (Overall Requests)}
% \phantomsection
% \bookmark[dest=meta_reviewer, level=1]{Meta Reviewer}

% {
% \hypertarget{meta_reviewer}{}



% %%% Meta Reviewer 1.1 subsection %%%
% \subsection{Discuss and evaluate the overhead in memory consumption. [Reviewer 5D1]}
% {
% %%% Meta Reviewer 1.1 subsection %%%

% Thank you for the request on memory usage analysis.
% In \figref{memory_analysis} and \revref{MR1} (p.10, left), we analyzed how efficient \thiswork is on memory usage and how expansion-aware sampling mitigates the neighbor explosion in deep GNNs (\figref{memory_analysis}a).
% Additionally, we showed that \thiswork can handle large graphs which the full-graph training cannot by transitioning to mini-batch training using \cobatch. \thiswork tries to use limited memory as efficiently as possible, especially when the graph is too large to be handled by the full-graph training (\figref{memory_analysis}b).

% }


% }

%%% Reviewer 1 Section %%%

% \vspace{3mm}
\setcounter{section}{0}
\section*{For All Reviewers}
\phantomsection
\bookmark[dest=areviewer, level=1]{All Reviewers}
\setcounter{subsection}{0}

{
\hypertarget{All Reviewers}{}

\subsection{D1: BFS and CC}
    We have optimized our implementations for BFS and CC, which allowed us to reduce both kernel computation and communication time. Because this brings a significant change to the benchmark results, we have replaced prior results with new ones on \figref{eval:benchmark}, and made necessary changes accordingly. We apologize for the confusion.
}

\subsection{D1: CPU baselines}
    W
}



%%% Reviewer 1 Section %%%

% \vspace{3mm}
\setcounter{section}{1}
\section*{For Reviewer \#1}
\phantomsection
\bookmark[dest=reviewer1, level=1]{Reviewer \#1}
\setcounter{subsection}{0}

{
\hypertarget{reviewer1}{}

\subsection{D1: Justification of Using PIM-Enabled DIMMs}
% Thank you for the suggestion. 
We added CPU baselines to \figref{@@} to demonstrate the high-performing PIM-enabled DIMMs.
The PIM baseline reflects the difficulty of fully utilizing PIM-enabled DIMM to outperform the CPU baseline due to its slow communication, especially for communication-heavy baselines such as @@ and @@. 
Despite this, \thiswork achieves @@ speedup compared to the PIM-enabled DIMM baseline due to effective communication.

\subsection{D2: Using PEs to Accelerate Computation}
% We apologize for the confusion. 
In \figref{eval:benchmark}, for PIM-enabled DIMM baseline and \thiswork, `Compute' represents the portion of execution time on computation on PEs. 
\SY{Is the following necessary?}
To avoid additional confusion, we use different color-coding for computation on the CPU and PIM-enabled DIMMs in \figref{eval:benchmark}.

\subsection{D2: \thiswork with Multi-Host Environment}
% Experimental results - Utilize dual-socket for multi-host environment experiment.
% Thank you for the suggestion. 
\thiswork can be applied to multi-host environments by adding another step of communication between multiple hosts while fully utilizing \thiswork's design. 
We added new experimental results in \figref{@@} by emulating the multi-host environment using two processes allocated to different sockets. 
We also share the expected performance of a multi-host environment with different communication standards. 
}


%%% Reviewer 2 Section %%%

% \vspace{3mm}
\setcounter{section}{2}
\section*{For Reviewer \#2}
\phantomsection
\bookmark[dest=reviewer2, level=1]{Reviewer \#2}
\setcounter{subsection}{0}

{
\hypertarget{reviewer2}{}

\subsection{D1: \thiswork with Other PIM Architectures}
Section~\ref{sec:discussion:otherpimarch} and Figure~\ref{fig:discussion:otherpimarch} are newly added on page~12.
This section explores the applicability of \thiswork{} for other PIM architectures. 
We explain in detail that as long as certain communication paths rely on the host, \thiswork's motivation and design can still give insight, albeit implementation details differ. 
\begin{comment}
They show how \thiswork{} is implemented on two alternative real-world PIM architectures: Samsung HBM-PIM~\cite{hbmpim} and Samsung AxDIMM~\cite{axdimm}. 
It is demonstrated that, notwithstanding the diverse characteristics of these PIM architectures, \thiswork{} consistently exhibits significant bandwidth improvements for \hl{all} categories of collective communication primitives on those architectures.
\end{comment}


\subsection{D2: Replacing Vector Instructions with Intel DSA}
%Experimental results - to compare data modulation performance of AVX512 with intel DSA, 
% Thank you for the suggestion. 
While DSA can alleviate the host's memory management burden, the current version does not include the necessary functions for data modulation (e.g. shifting). 
However, once these requirements are met, we expect DSA could accelerate data modulation even more. 

\subsection{D3: Implementing Collective Communications with CXL NMP}
% Discussion - yes the same techniques will work in CXL NMPs too. detailed explanation to add later
\SY{Same with R2D1}


\subsection{D4: Separating Performance Benefits between PIM-Enabled DIMMs and \thiswork}
\SY{Same with R1D1} 
%divide into PIM-friendly and PIM-unfriendly, show most applications in the benchmark are Faster than CPU baseline (reference to figure), explanation on BFS and CC

}

%%% Reviewer 3 Section %%%

% \vspace{3mm}
\setcounter{section}{3}
\section*{For Reviewer \#3}
\phantomsection
\bookmark[dest=reviewer3, level=1]{Reviewer \#3}
\setcounter{subsection}{0}

{
\hypertarget{reviewer3}{}

\subsection{D1: Figures' Font size}
% We apologize.
We increased the font size of figures in {\color{olivegreen}green boxes} labeled as @@.

\subsection{D2: Non-PIM Baseline}
\SY{Same with R1D1}
%divide into PIM-friendly and PIM-unfriendly, show most applications in the benchmark are Faster than CPU baseline (reference to figure), explanation on BFS and CC

\subsection{D3: Optimization compared to SimplePIM~\cite{simplepim}}
%Discussion - Simplepim's implementations are unoptimized in that the three schemes (avoid transpose, evade hostmem, pim-assisted reordering) in the paper are not applied. We applied the 3 schemes in the library implementations. Primitives already implemented in SimplePIM also benefit performance-wise in our new implementation. (See figure 14, base is SimplePIM)
% We apologize for the confusion. 
The main difference of \thiswork compared to SimplePIM is three-fold: optimizing collective communication operations as shown in \tblref{techniques}, allowing multi-dimensional collective communication with virtual hypercube model, and supporting additional primitives (AA, RS, Re) as in \tblref{prior}.  
Performance comparison between SimplePIM and \thiswork can be located in \figref{eval:centprim}.

}

%%% Reviewer 4 Section %%%

% \vspace{3mm}
\setcounter{section}{4}
\section*{For Reviewer \#4}
\phantomsection
\bookmark[dest=reviewer4, level=1]{Reviewer \#4}
\setcounter{subsection}{0}

{
\hypertarget{reviewer4}{}
% We apologize for any confusion and would like to clarify them below. 
% We also appreciate any suggestions made. 

\subsection{D1: Comparison with Hierarchy-Aware Approaches}
\begin{comment}
Thank you for your comment on the potential effects of other hierarchy-aware approaches.
Section~\ref{} and Figure~\ref{} are newly added on page~X.
This section shows the effects of the hierarchy-aware approach based on the DIMMs' memory architecture.
It is shown that performing collective communication concerning the DIMM's memory hierarchy (e.g., banks, chips, and ranks) has a negligible impact on the bandwidth of \thiswork. 
\end{comment}
% Thank you for the suggestion.
We tested additional topologies (ring, tree) within the PIM-enabled DIMM in @@.
Compared to other baselines, \thiswork achieved the highest performance due to using the entangled group as the smallest effective unit for flexible communication. 

\subsection{D2: Clarifying Baseline Measurement}

% We apologize for the confusion and appreciate the advice on improving the clarity of the baseline system configuration setups.
Both SimplePIM~\cite{simplepim} and \thiswork were evaluated for performance on a UPMEM-enabled system.
To fix the misleading description, %of the CPIstack method in \secref{eval:benchmark}, 
we revised the following sections:

\begin{itemize}
    \item \secref{eval:setup}: We explicitly state that all baselines and \thiswork is implemented and measured on a real system. 
    \item \secref{eval:benchmark}: For \figref{eval:benchmark} breakdown, we did not use CPIstack-related methods. We measured the execution time of each portion on a real system. Thus, we remove this description. 
    \item \secref{eval:ablation}: For \figref{eval:Primitive_breakdown}, we used a CPIstack-like method on a real system to breakdown highly overlapping portions. We added the related description accordingly. 
\end{itemize}

\subsection{D3: Applying \thiswork to Different Communication Networks on PIM-Enabled DIMMs and future generation PIM}
%comm. still needed. ex)HBM PIM
\SY{Same with R2D1}

}

%%% Reviewer 5 Section %%%

% \vspace{3mm}
\setcounter{section}{5}
\section*{For Reviewer \#5}
\phantomsection
\bookmark[dest=reviewer5, level=1]{Reviewer \#5}
\setcounter{subsection}{0}

{
\hypertarget{reviewer5}{}

% We apologize for any confusion and would like to clarify them below. 

\subsection{D1: Gather/Broadcast Latencies in the Benchmarks}

% Clarify \& modify figure 
%We apologize for the confusion. 
As in \tblref{baselines}, DLRM and GNN AR\&AG include Gather, and DLRM, BFS and CC include Broadcast, albeit a small portion. 
%We have increased the height of \figref{eval:benchmark} to provide a clearer view of the two primitives. 
We added the exact portion of both primitives in evaluation @@. 

\subsection{D2: PE-Assisted Reordering Overhead}
% Clarify - reordering overhead is already included in each primitive execution time.
%We apologize for the confusion.
The portion in @@ labeled "PE-side modulation" represents the overhead introduced by PE-assisted reordering.
For example, @@s host-side modulation is replaced with @@s PE-side modulation in @@.
Reordering in PE is done by @@.

\subsection{D3: Bandwidth Requirements of Broadcast}
%% Clarify - fig 14's results are performance measurements of primitives on our system setup. It doesn't necessarily mean that broadcast requires very high bandwidth, but rather that it shows the highest performance compared to other primitives in the same setup.
%We apologize for the confusion. 
\figref{eval:centprim}'s y-axis does not imply bandwidth requirements but the performance of the primitive.
We replaced the y-axis label `bandwidth' to `throughput' for figures labeled as @@.


\subsection{D4: PE-Assisted Reordering in Reduce Scatter}
%% Clarify - Reordering enables storing data with different destinations in one vector register. After in-register rotation is performed, data with the same destination is located in the same index of the vector register. Finally, inter-vector register addition is performed for results.
%We apologize for the confusion. 
To utilize AVX's vector sum operations, values to be added must reside in different registers. 
%Thus, if PE-assisted reordering were not used, the host would have to redistribute the data within the host memory and then read the redistributed data back to separate vector registers, causing additional memory access overhead.
Without PE-assisted reordering, target values would reside in the same vector, requiring the host to read\&redistribute data to different vectors for summation.
PE-assisted reordering allows target values to reside in different vectors without any additional actions, minimizing unnecessary memory access overhead.
This applies to both ReduceScatter and AllReduce.
}

}




==> cover_letter_backups/240222_index_backup_single_page.tex <==
\bookmark[level=0]{Revision document}
{

\begin{center}
{\large{\textbf{\textsc{Response to Reviewer Comments}}}}
\end{center}

% \vspace{1mm}


\begin{center}
\setlength{\fboxrule}{1pt}
\fbox{\begin{minipage}{0.95\columnwidth} 
We sincerely thank the reviewers for their time and valued comments, and apologize for any confusion. We have faithfully revised our paper and addressed each reviewer's comments below with much appreciation. All the revised texts are written in {\color{olivegreen}green color} with {\color{magenta}magenta markers}. %{\color{magenta}{R$i$:$k$, MR1-MR6}} around them. 
%Please refer to the overall requests below with \underline{hyperlinks} to them. 
%Note that the term `Reviewer $i$D$k$' means the discussion point $k$ from the reviewer $i$.
\end{minipage}} 
\end{center}

% %%% Meta Reviewer Section %%%
     
% \setcounter{section}{1}
% \section*{For the Meta-Reviewer (Overall Requests)}
% \phantomsection
% \bookmark[dest=meta_reviewer, level=1]{Meta Reviewer}

% {
% \hypertarget{meta_reviewer}{}



% %%% Meta Reviewer 1.1 subsection %%%
% \subsection{Discuss and evaluate the overhead in memory consumption. [Reviewer 5D1]}
% {
% %%% Meta Reviewer 1.1 subsection %%%

% Thank you for the request on memory usage analysis.
% In \figref{memory_analysis} and \revref{MR1} (p.10, left), we analyzed how efficient \thiswork is on memory usage and how expansion-aware sampling mitigates the neighbor explosion in deep GNNs (\figref{memory_analysis}a).
% Additionally, we showed that \thiswork can handle large graphs which the full-graph training cannot by transitioning to mini-batch training using \cobatch. \thiswork tries to use limited memory as efficiently as possible, especially when the graph is too large to be handled by the full-graph training (\figref{memory_analysis}b).

% }


% }

%%% Reviewer 1 Section %%%

% \vspace{-3mm}
\setcounter{section}{0}
\section*{For All Reviewers}
\phantomsection
\bookmark[dest=areviewer, level=1]{All Reviewers}
\setcounter{subsection}{0}

{
\hypertarget{All Reviewers}{}

\subsection{Comparison with CPU-only baselines}

Thank you for the suggestion. We added comparisons with CPU-only baselines (i.e., without PIM) to \figref{eval:cpu_comp} to demonstrate the high-performing PIM-enabled DIMMs.
While doing so, we made some optimizations to the benchmark implementations, and updated the results on \figref{eval:benchmark}.
The PIM baseline reflects the difficulty of fully utilizing PIM-enabled DIMM to outperform the CPU baseline due to its slow communication, especially for communication-heavy baselines such as CC. 
Despite this, \thiswork achieves a geomean speedup of 1.99 compared to the PIM-enabled DIMM baseline due to effective communication.


\subsection{Applying \thiswork to Other PIM Architectures}

Section~\ref{sec:discussion:otherpimarch} and \figref{disc:diffhard} are newly added. %on page~12.
This section explores the applicability of \thiswork{} for other PIM architectures. 
We explain in detail that as long as certain communication paths rely on the host, \thiswork's motivation and design can still give insight, albeit implementation details slightly differ.  
\begin{comment}
They show how \thiswork{} is implemented on two alternative real-world PIM architectures: Samsung HBM-PIM~\cite{hbmpim} and Samsung AxDIMM~\cite{axdimm}. 
It is demonstrated that, notwithstanding the diverse characteristics of these PIM architectures, \thiswork{} consistently exhibits significant bandwidth improvements for \hl{all} categories of collective communication primitives on those architectures.
\end{comment}


}



%%% Reviewer 1 Section %%%

% \vspace{3mm}
\setcounter{section}{1}
\section*{For Reviewer \#1}
\phantomsection
\bookmark[dest=reviewer1, level=1]{Reviewer \#1}
\setcounter{subsection}{0}

{
\hypertarget{reviewer1}{}

% \subsection{Justification of Using PIM-Enabled DIMMs}
% Thank you for the suggestion. 


\subsection{Using PEs to Accelerate Computation}
% We apologize for the confusion. 
In \figref{eval:benchmark}, for PIM-enabled DIMM baseline and \thiswork, `Compute' represents the portion of execution time on computation on PEs. 
To avoid additional confusion, we use different color-coding for computation on the CPU and PIM-enabled DIMMs in \figref{eval:benchmark}.

\subsection{\thiswork with Multi-Host Environment}
% Experimental results - Utilize dual-socket for multi-host environment experiment.
% Thank you for the suggestion. 
\thiswork can be % applied to multi-host environments 
extended by adding another step of communication between multiple hosts while utilizing \thiswork's design. 
We added new experimental results in \figref{eval:multihost_hier} by emulating the multi-host environment with different communication standards using two processes allocated to different sockets. 
% We also share the expected performance of a multi-host environment with different communication standards. 
}


%%% Reviewer 2 Section %%%

% \vspace{3mm}
\setcounter{section}{2}
\section*{For Reviewer \#2}
\phantomsection
\bookmark[dest=reviewer2, level=1]{Reviewer \#2}
\setcounter{subsection}{0}

{
\hypertarget{reviewer2}{}

% \subsection{\thiswork with Other PIM Architectures}



\subsection{Replacing Vector Instructions with Intel DSA}
%Experimental results - to compare data modulation performance of AVX512 with intel DSA, 
% Thank you for the suggestion. 
While DSA can alleviate the host's memory management burden, the current version does not include the necessary functions for data modulation (e.g. shifting). 
Once these requirements are met, we expect DSA could additionally accelerate data modulation. 

% \subsection{Implementing Collective Communications with CXL NMP}
% % Discussion - yes the same techniques will work in CXL NMPs too. detailed explanation to add later
% \SY{Same with R2D1}


% \subsection{Separating Performance Benefits between PIM-Enabled DIMMs and \thiswork}
% \SY{Same with R1D1} 
% divide into PIM-friendly and PIM-unfriendly, show most applications in the benchmark are Faster than CPU baseline (reference to figure), explanation on BFS and CC

}

%%% Reviewer 3 Section %%%

% \vspace{3mm}
\setcounter{section}{3}
\section*{For Reviewer \#3}
\phantomsection
\bookmark[dest=reviewer3, level=1]{Reviewer \#3}
\setcounter{subsection}{0}

{
\hypertarget{reviewer3}{}

\subsection{Figures' Font size}
% We apologize.
We increased the figures' font size labeled as @@.

% \subsection{Non-PIM Baseline}
% \SY{Same with R1D1}
%divide into PIM-friendly and PIM-unfriendly, show most applications in the benchmark are Faster than CPU baseline (reference to figure), explanation on BFS and CC

\subsection{Optimization compared to SimplePIM~\cite{simplepim}}
%Discussion - Simplepim's implementations are unoptimized in that the three schemes (avoid transpose, evade hostmem, pim-assisted reordering) in the paper are not applied. We applied the 3 schemes in the library implementations. Primitives already implemented in SimplePIM also benefit performance-wise in our new implementation. (See figure 14, base is SimplePIM)
% We apologize for the confusion. 
The main difference of \thiswork compared to SimplePIM is three-fold: optimizing collective communication (\tblref{techniques}), allowing multi-dimensional collective communication with virtual hypercube model, and supporting additional primitives AA, RS, and Re (\tblref{prior}).  
Detailed performance comparison is in \figref{eval:centprim}.

}

%%% Reviewer 4 Section %%%

% \vspace{3mm}
\setcounter{section}{4}
\section*{For Reviewer \#4}
\phantomsection
\bookmark[dest=reviewer4, level=1]{Reviewer \#4}
\setcounter{subsection}{0}

{
\hypertarget{reviewer4}{}
% We apologize for any confusion and would like to clarify them below. 
% We also appreciate any suggestions made. 

\subsection{Clarifying Baseline Measurement}

% We apologize for the confusion and appreciate the advice on improving the clarity of the baseline system configuration setups.
Sorry for the confusion. \ul{All measurements are made on a real system}, including both the baseline and \thiswork. We did not use simulators for any experiments in the paper. % were evaluated for performance on a UPMEM-enabled system.
To fix the misleading description, %of the CPIstack method in \secref{eval:benchmark}, 
we revised the following sections:

\begin{itemize}
    \item \secref{eval:setup}: We explicitly state that all baselines and \thiswork is implemented and measured on a real system. 
    \item \secref{eval:benchmark}: For \figref{eval:benchmark}, we did not use CPIstack-like method. 
    %We measured the execution time of each portion on a real system. 
    Thus, we removed this description. 
    \item \secref{eval:ablation}: For \figref{eval:Primitive_breakdown}, we used a CPIstack-like method on a real system to breakdown highly overlapping portions. We added the related description accordingly. 
\end{itemize}


\subsection{Comparison with Hierarchy-Aware Approaches}
\begin{comment}
Thank you for your comment on the potential effects of other hierarchy-aware approaches.
Section~\ref{} and Figure~\ref{} are newly added on page~X.
This section shows the effects of the hierarchy-aware approach based on the DIMMs' memory architecture.
It is shown that performing collective communication concerning the DIMM's memory hierarchy (e.g., banks, chips, and ranks) has a negligible impact on the bandwidth of \thiswork. 
\end{comment}
% Thank you for the suggestion.
We tested additional topologies (ring, tree) within the PIM-enabled DIMM in \figref{eval:multihost_hier}.
Compared to other baselines, \thiswork achieved the highest performance due to using the entangled group as the smallest effective unit for flexible communication. 

% \subsection{Applying \thiswork to Different Communication Networks on PIM-Enabled DIMMs and future generation PIM}
% %comm. still needed. ex)HBM PIM
% \SY{Same with R2D1}

}

%%% Reviewer 5 Section %%%

% \vspace{3mm}
\setcounter{section}{5}
\section*{For Reviewer \#5}
\phantomsection
\bookmark[dest=reviewer5, level=1]{Reviewer \#5}
\setcounter{subsection}{0}

{
\hypertarget{reviewer5}{}

% We apologize for any confusion and would like to clarify them below. 

\subsection{Gather/Broadcast Latencies in the Benchmarks}

% Clarify \& modify figure 
%We apologize for the confusion. 
As in \tblref{baselines}, %DLRM and GNN AR\&AG include Gather, and DLRM, BFS and CC include Broadcast
multiple benchmarks include both Ga and Bc, albeit a small portion. 
%We have increased the height of \figref{eval:benchmark} to provide a clearer view of the two primitives. 
We added the exact portion of both primitives in evaluation @@. 

\subsection{PE-Assisted Reordering Overhead}
% Clarify - reordering overhead is already included in each primitive execution time.
%We apologize for the confusion.
The portion in \figref{eval:Primitive_breakdown} labeled "PE-side modulation" represents the overhead introduced by PE-assisted reordering.
For example, @@s host-side modulation is replaced with @@s PE-side modulation in @@.
Reordering in PE is done by @@. \NS{PE side modulation is very small(about 1~3\% (30ms) in the graph}

\subsection{Bandwidth Requirements of Broadcast}
%% Clarify - fig 14's results are performance measurements of primitives on our system setup. It doesn't necessarily mean that broadcast requires very high bandwidth, but rather that it shows the highest performance compared to other primitives in the same setup.
%We apologize for the confusion. 
\figref{eval:centprim}'s y-axis does not imply bandwidth requirements but the performance of the primitive.
We replaced the y-axis label `bandwidth' to `throughput' for figures labeled as @@.


\subsection{PE-Assisted Reordering in Reduce Scatter}
%% Clarify - Reordering enables storing data with different destinations in one vector register. After in-register rotation is performed, data with the same destination is located in the same index of the vector register. Finally, inter-vector register addition is performed for results.
%We apologize for the confusion. 
To use AVX's vector sum operations, % values to be added 
target values must reside in different registers. 
%Thus, if PE-assisted reordering were not used, the host would have to redistribute the data within the host memory and then read the redistributed data back to separate vector registers, causing additional memory access overhead.
% Without PE-assisted reordering, target values would reside in the same vector, requiring the host to read\&redistribute data to different vectors for summation.
% Thus, without PE-assisted reordering, the host has to redistribute data to different vectors using memory. 
PE-assisted reordering efficiently sets this up without additional actions (i.e., host moving data to different registers using memory), minimizing overhead.
% This applies to both ReduceScatter and AllReduce.
}

}




==> index.tex <==
\bookmark[level=0]{Revision document}
{

\begin{center}
{\large{\textbf{\textsc{Response to Reviewer Comments}}}}
\end{center}

% \vspace{1mm}


\begin{center}
\setlength{\fboxrule}{1pt}
\fbox{\begin{minipage}{0.95\columnwidth} 
We sincerely thank the reviewers for their time and valued comments. We have faithfully revised our paper and addressed each reviewer's comments below with much appreciation. All the revised texts are written in {\color{olivegreen}green color}. 
%We color-coded each reviewer as 
%{\color{brown}Rev A}, {\color{orange}Rev B}, {\color{magenta}Rev C}, {\color{cyan}Rev D}, {\color{violet}Rev E}.
%{\color{magenta}{R$i$:$k$, MR1-MR6}} around them. 
%Please refer to the overall requests below with \underline{hyperlinks} to them. 
%Note that the term `Reviewer $i$D$k$' means the discussion point $k$ from the reviewer $i$.
\end{minipage}} 
\end{center}

% %%% Meta Reviewer Section %%%
     
% \setcounter{section}{1}
% \section*{For the Meta-Reviewer (Overall Requests)}
% \phantomsection
% \bookmark[dest=meta_reviewer, level=1]{Meta Reviewer}

% {
% \hypertarget{meta_reviewer}{}



% %%% Meta Reviewer 1.1 subsection %%%
% \subsection{Discuss and evaluate the overhead in memory consumption. [Reviewer 5D1]}
% {
% %%% Meta Reviewer 1.1 subsection %%%

% Thank you for the request on memory usage analysis.
% In \figref{memory_analysis} and \revref{MR1} (p.10, left), we analyzed how efficient \thiswork is on memory usage and how expansion-aware sampling mitigates the neighbor explosion in deep GNNs (\figref{memory_analysis}a).
% Additionally, we showed that \thiswork can handle large graphs which the full-graph training cannot by transitioning to mini-batch training using \cobatch. \thiswork tries to use limited memory as efficiently as possible, especially when the graph is too large to be handled by the full-graph training (\figref{memory_analysis}b).

% }


% }

%%% Reviewer 1 Section %%%

% \vspace{-3mm}
\setcounter{section}{0}
\section*{For All Reviewers}
\phantomsection
\bookmark[dest=areviewer, level=1]{All Reviewers}
\setcounter{subsection}{0}

{
\hypertarget{areviewer}{}

\subsection{Comparison with CPU-only system [{\color{brown}Rev A}, {\color{orange}Rev B}, {\color{magenta}Rev C}]}\vspace{-1mm}

% Thank you for the suggestion. 
We agree with the reviewers that comparing the PID-Comm-enabled PIM with the CPU-only systems (i.e., without PIM) is important to further emphasize the significance and impact of \thiswork.
In the original submission, PID-Comm focuses on improving inter-PE communication, so we used the existing PIM kernels for the benchmarks. Since the performance of a PIM implementation depends on not only inter-PE communication but also the PIM kernel itself (e.g., PE utilization), we further optimized both PIM and CPU kernels of the benchmarks and compared them in this revised version.
Please find the results in \figref{eval:cpu_comp} and \secref{eval:cpu}. 
PIM baseline achieves 2.27\texttimes{} geomean speedup over the CPU-only system, and \thiswork achieves 4.07\texttimes{} geomean speedup.

%The PIM baseline reflects the difficulty of fully utilizing PIM-enabled DIMM to outperform the CPU-only system due to its slow communication, especially for communication-heavy baselines (e.g., CC). 

%We would like to also 
%Please note that we do not intend to take credit for PIM systems having speedup over CPU-only systems.
%As the reviewers stated, this serves the purpose of showing that the chosen benchmark applications are suitable for PIM.
% Despite this, \thiswork achieves a geomean speedup of 1.99 compared to the PIM-enabled DIMM baseline due to effective communication.


\subsection{Applying \thiswork to Other PIM Architectures/Systems [{\color{brown}Rev A}, {\color{orange}Rev B}, {\color{cyan}Rev D}]}\vspace{-1mm}

Unless all PEs share a communication medium (e.g., interconnect, shared buffer), \thiswork is still beneficial. %, albeit some modifications in the details.  
Newly added \secref{discussion:otherpimarch} explores \thiswork{}'s applicability to other architectures (multi-host, AxDIMM, HBM-PIM, and CXL-NMP) with results from multi-host settings in \figref{eval:multihost_hier}(b).


\subsection{Hardware-side Implications [{\color{magenta}Rev C}, {\color{cyan}Rev D}]}\vspace{-1mm}
Thank you. 
\thiswork only involves software techniques to be a ready-to-use solution. 
However, we agree that adding hardware-side insights would strengthen the paper. 
%While hardware-side solutions are out of \thiswork's scope, 
In \secref{discussion:hw}, we discuss possible hardware solutions for offloading host involvement and enabling inter-PE paths.
%We also discuss extending to different PIM architectures in \secref{discussion:otherpimarch}.
%We expect both to be easily integrated since \thiswork focuses on software solutions. %, providing flexibility and compatibility. 
}



%%% Reviewer 1 Section %%%


\setcounter{section}{1}
\section*{For {\color{brown}Reviewer A}}

\phantomsection
\bookmark[dest=reviewerA, level=1]{Reviewer A}
\setcounter{subsection}{0}


\hypertarget{reviewerA}{}

% \subsection{Justification of Using PIM-Enabled DIMMs}
% Thank you for the suggestion. 


\subsection{Using PEs to Accelerate Computation}\vspace{-1mm}
% We apologize for the confusion. 
PIM baseline and \thiswork \ul{both use PEs to accelerate computation}.
Please see the added description of this in \secref{apps}.
We also modified label `Compute' to `Kernel' in \figref{eval:benchmark} for clarity. 

% To avoid additional confusion, we use different color-coding for computation on the CPU and PIM-enabled DIMMs in \figref{eval:benchmark}.

\subsection{Extending \thiswork to Multi-Host Environments}\vspace{-1mm}
% Experimental results - Utilize dual-socket for multi-host environment experiment.
% Thank you for the suggestion. 
\thiswork can be % applied to multi-host environments 
extended to multi-host environments by adding another step of communication. % between hosts while utilizing \thiswork's design within a single host. 
We added new results in \figref{eval:multihost_hier}(b) and \thiswork still shows a large speedup. % by emulating the multi-host environment with different communication standards using two processes in a hierarchical manner. 
% We also share the expected performance of a multi-host environment with different communication standards. 



%%% Reviewer 2 Section %%%

% \vspace{3mm}
\setcounter{section}{2}
\section*{For {\color{orange}Reviewer B}}
\phantomsection
\bookmark[dest=reviewerB, level=1]{Reviewer B}
\setcounter{subsection}{0}


\hypertarget{reviewerB}{}

% \subsection{\thiswork with Other PIM Architectures}



\subsection{Replacing General Purpose Cores with Intel DSA}\vspace{-1mm}
%Experimental results - to compare data modulation performance of AVX512 with intel DSA, 
% Thank you for the suggestion. 

Thank you for the great idea. The host-side overhead could be greatly alleviated if there is a dedicated accelerator such as DSA.
%currently does not include the necessary functions for data modulation, thus it is not possible to offload host-side modulations.  
Even though the current version of DSA lacks the necessary computational features for performing target collective communications, we expect adding those features such as add, shift, and/or domain transfers to DSA could additionally accelerate \thiswork, as newly discussed in \secref{discussion:hw}.

% \subsection{Implementing Collective Communications with CXL NMP}
% % Discussion - yes the same techniques will work in CXL NMPs too. detailed explanation to add later
% \SY{Same with R2D1}


% \subsection{Separating Performance Benefits between PIM-Enabled DIMMs and \thiswork}
% \SY{Same with R1D1} 
% divide into PIM-friendly and PIM-unfriendly, show most applications in the benchmark are Faster than CPU baseline (reference to figure), explanation on BFS and CC



%%% Reviewer 3 Section %%%

% \vspace{3mm}
\setcounter{section}{3}
\section*{For {\color{magenta}Reviewer C}}
\phantomsection
\bookmark[dest=reviewerC, level=1]{Reviewer C}
\setcounter{subsection}{0}

{
\hypertarget{reviewerC}{}

\subsection{Figures' Font Size}\vspace{-1mm}
% We apologize.
Thank you. We modifed \figref{hypercube}, \figref{multiaxes}, \figref{pidcomm_apis} and \figref{dlrm}.

% \subsection{Non-PIM Baseline}
% \SY{Same with R1D1}
%divide into PIM-friendly and PIM-unfriendly, show most applications in the benchmark are Faster than CPU baseline (reference to figure), explanation on BFS and CC

\subsection{Difference with SimplePIM~\cite{simplepim}}\vspace{-1mm}

% The main difference of \thiswork compared to SimplePIM is three-fold: optimizing collective communication (\tblref{techniques}), allowing multi-dimensional collective communication with the virtual hypercube model, and supporting additional primitives AA, RS, and Re (\tblref{prior}).  
\figref{commlib}(a) shows SimplePIM's design. Unlike \thiswork, SimplePIM uses data modulation within host memory and calls domain transfer even for primitives without arithmetic operations. 
\thiswork's solutions for SimplePIM's inefficiencies are illustrated in \figref{commlib}(b)-(d).
In addition, SimplePIM does not support flexible communication groups and mandates that all PEs participate in communication.

}

%%% Reviewer 4 Section %%%

% \vspace{3mm}
\setcounter{section}{4}
\section*{For {\color{cyan}Reviewer D}}
\phantomsection
\bookmark[dest=reviewerD, level=1]{Reviewer D}
\setcounter{subsection}{0}

{
\hypertarget{reviewerD}{}
% We apologize for any confusion and would like to clarify them below. 
% We also appreciate any suggestions made. 

\subsection{Clarifying Baseline Measurement}\vspace{-1mm}

% We apologize for the confusion and appreciate the advice on improving the clarity of the baseline system configuration setups.
% We apologize for the confusion. 
\ul{All measurements are made on a real system}, including CPU, PIM baselines and \thiswork. We did not use simulators for any experiments in the paper. % were evaluated for performance on a UPMEM-enabled system.
To fix the misleading description, %of the CPIstack method in \secref{eval:benchmark}, 
we explicitly stated in \secref{eval:setup} that all baselines and \thiswork are evaluated on a real system. 
%we revised the following sections:

% \begin{itemize}
%     \item \secref{eval:setup}: We explicitly state that all baselines and \thiswork is implemented and measured on a real system. 
%     \item \secref{eval:benchmark}: For \figref{eval:benchmark}, we did not use CPIstack-like method. 
%     %We measured the execution time of each portion on a real system. 
%     Thus, we removed this description. 
%     \item \secref{eval:ablation}: For \figref{eval:Primitive_breakdown}, we used a CPIstack-like method on a real system to breakdown highly overlapping portions. We added the related description accordingly. 
% \end{itemize}


\subsection{Comparison with Hierarchy-Aware Approaches}\vspace{-1mm}
\begin{comment}
Thank you for your comment on the potential effects of other hierarchy-aware approaches.
Section~\ref{} and Figure~\ref{} are newly added on page~X.
This section shows the effects of the hierarchy-aware approach based on the DIMMs' memory architecture.
It is shown that performing collective communication concerning the DIMM's memory hierarchy (e.g., banks, chips, and ranks) has a negligible impact on the bandwidth of \thiswork. 
\end{comment}
% Thank you for the suggestion.
We tested additional collective communication algorithms using other topologies (ring, tree) in \figref{eval:multihost_hier}(a).
\thiswork achieves 2.05\texttimes{} improvement compared to the fastest ring algorithm thanks to using the flexible hypercube topology. %for flexible communications. 

% \subsection{Applying \thiswork to Different Communication Networks on PIM-Enabled DIMMs and future generation PIM}
% %comm. still needed. ex)HBM PIM
% \SY{Same with R2D1}

}

%%% Reviewer 5 Section %%%

% \vspace{3mm}
\setcounter{section}{5}
\section*{For {\color{violet}Reviewer E}}
\phantomsection
\bookmark[dest=reviewerE, level=1]{Reviewer E}
\setcounter{subsection}{0}

{
\hypertarget{reviewerE}{}

% We apologize for any confusion and would like to clarify them below. 
\subsection{Gather/Broadcast Latencies in the Benchmarks}\vspace{-1mm}

% Clarify \& modify figure 
%We apologize for the confusion. 
%DLRM and GNN AR\&AG include Gather, and DLRM, BFS and CC include Broadcast
Multiple benchmarks include both Gather and Broadcast (refer to \tblref{baselines}), albeit a small portion. 
%We have increased the height of \figref{eval:benchmark} to provide a clearer view of the two primitives. 
We added the maximum portion of both primitives in \secref{eval:benchmark}. 
For better performance estimation of the two primitives, we have also reported their throughput separately in \figref{eval:centprim}.%\secref{eval:collcomm}.

\subsection{PE-Assisted Reordering Details}\vspace{-1mm}
%% Method
PE-assisted reordering is done by incrementally shifting data using WRAM, newly described in \secref{design:pr}.
% We added a detailed description in \secref{design:pr}.
%
%% Overhead
As multiple PEs reorder the data in parallel, they are capable of faster reordering compared to host processors.
In \figref{eval:Primitive_breakdown}, the 4.5\% overhead of PE-assisted reordering (`PE-side Modulation') replaces an average of 30\% overhead of host-side modulation.
We added detailed description in \secref{eval:ablation}.
% The portion in \figref{eval:Primitive_breakdown} labeled "PE-side modulation" represents the overhead introduced by PE-assisted reordering.
% For example, @@s host-side modulation is replaced with @@s PE-side modulation in @@.
% Reordering in PE is done by @@. 

\subsection{Bandwidth Requirements of Broadcast}\vspace{-1mm}
%% Clarify - fig 14's results are performance measurements of primitives on our system setup. It doesn't necessarily mean that broadcast requires very high bandwidth, but rather that it shows the highest performance compared to other primitives in the same setup.
%We apologize for the confusion. 
\figref{eval:centprim}'s y-axis \ul{does not imply bandwidth requirements but the performance (throughput) of the primitives}.
We replaced the y-axis label from `bandwidth' to `throughput' for  \figref{eval:centprim}, \figref{eval:ablation}, \figref{eval:datasize}, \figref{eval:numdpus}, and \figref{eval:hypercube}.


\subsection{Benefits of Using PE-Assisted Reordering in ReduceScatter}\vspace{-1mm}
Without PE-assisted reordering,
%If PE-assisted reordering (PR) is not used in ReduceScatter, the reduction cannot benefit from SIMD instructions. 
%For example, in \figref{commlibprim}(b), a0,a1,a2, and a3 would be placed within a single vector register. 
target values will reside in a single register, requiring horizontal reduction.
However, horizontal reduction in AVX (and many other SIMD ISAs) is inefficient as it must be done with multiple costly instructions. 
On the other hand, in-register modulation allows for vertical reduction, which can be done with a single instruction per vector register.
We added related description in \secref{design:others:RS}.
\begin{comment}
Target values must reside in different registers to use AVX's vector sum operations. 
PE-assisted reordering efficiently sets this up without host memory access, minimizing overhead.
\end{comment}
}

}




==> multihost-backup.tex <==

\subsection{\rev{Performance on Multi-Host Collectives}}
\rev{
In this section, we assess the compatibility of \thiswork in multi-host environments in \cref{fig:eval:multihost_hier}(a) by doing a breakdown study.
We compare the performance of \thiswork in two different environments, single-host dual-socket and an emulated real-world scenario of hosts connected with @@ and @@. 
To run \thiswork on a multi-host environment, we added an additional code block using MPI~\cite{@@} to send and receive intermediate results between processes on different hosts. 
Appropriate changes to the implementations were made accordingly.
In the emulated multi-host environment, the execution time increases from @@ to @@ due to communication between hosts and additional host memory access time.
However, it is clear that \thiswork is effectively removing communication overhead in PIM-enabled DIMMs compared to the PIM baseline in an emulated multi-host scenario, thus demonstrating that \thiswork can indeed be expanded to multi-host environments and still benefit from its designs.
%In multi-host dual-socket, communication between hosts becomes the main bottleneck, increasing the execution time from @@ to @@ in @@. 
%Additionally, by emulating real-world scenarios of @@ and @@, we can see that this bottleneck can be reduced to @@, effectively demonstrating that \thiswork can indeed be expanded to multi-host environments and still benefit from its designs.

} 



Although adjacent communication PEs can benefit from this, there are situations where host access is unavoidable, such as when communicating between PEs in different channels or through CXL switches.
The concepts presented in \thiswork can also address the need for host access in such scenarios.
The only case where \thiswork's ideas become inapplicable is with an architecture where each PE has direct access to other PEs. 
However, this seems to be an unlikely scenario in the foreseeable future unless there is a breakthrough that significantly reduces the cost and power requirements of such extensively interconnected hardware.

Furthermore, we contend that while the specifics of implementation and optimization may vary, the challenges and solutions presented by \thiswork can offer compelling insights for addressing similar issues in architectures from both categories.
Communication within these architectures is heavily influenced by the design of the hardware, and any form of communication inherently adds overhead or necessitates additional computation.
The former can benefit from \thiswork's virtual hypercube communication model, which facilitates flexible communication with minimal constraints on efficiency.
The latter can leverage \thiswork's performance optimization techniques, which redistribute computational operations for communication to the host and PEs. 

==> tables/accuracy.tex <==
\begin{table}[]
    \centering
    \resizebox{\columnwidth}{!}
    {
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{cccccccccc}
    \toprule
         Dataset& \multicolumn{3}{c}{ogbn-arxiv}  & \multicolumn{3}{c}{ogbn-products} & \multicolumn{3}{c}{Reddit} \\
         \cmidrule(lr){2-4}
         \cmidrule(lr){5-7}
        \cmidrule(lr){8-10}
         \#Layers& 3 & 28 & 56 & 3 & 28 & 56 & 3 & 28 & 56 \\
         % \cmidrule(lr){2-3}
         % \cmidrule(lr){4-5}
         % \cmidrule(lr){6-7}
         % \cmidrule(lr){8-9}
         % \cmidrule(lr){10-11}
         % \cmidrule(lr){12-13}
         % \cmidrule(lr){14-15}
         % \cmidrule(lr){16-17}
         % \cmidrule(lr){18-19}
         % & \makecell{Acc. (\%)} &\makecell{Acc. (\%)}  & \makecell{Acc. (\%)}  &  \makecell{Acc. (\%)}  &\makecell{Acc. (\%)}  & \makecell{Acc. (\%)} &  \makecell{Acc. (\%)}  &\makecell{Acc. (\%)} & \makecell{Acc. (\%)} \\
         \midrule
         FG & 70.72 & 70.44 & 70.40 & 76.01 & 75.50 & 74.58 & 96.20 & 96.13 & 96.39  \\
         \thiswork  & 70.57 & 70.50 & 70.68 & 75.44 & 75.21 & 74.88 & 96.06 & 96.14 & 96.08  \\
        \bottomrule
    \end{tabular}
    }
    \caption{Accuracy (\%) of the full-graph training and \thiswork} \label{tab:acc_compare}
\end{table}

==> tables/accuracy_speedup.tex <==
\begin{table*}[]
    \centering
    \label{tab:acc_compare}
    \resizebox{\textwidth}{!}
    {
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{ccccccccccccccccccc}
    \toprule
         \multirowcell{3}{Method}& \multicolumn{6}{c}{ogbn-arxiv}  & \multicolumn{6}{c}{ogbn-products} & \multicolumn{6}{c}{Reddit} \\
         \cmidrule(lr){2-7}
         \cmidrule(lr){8-13}
        \cmidrule(lr){14-19}
         & \multicolumn{2}{c}{3-layer} & \multicolumn{2}{c}{28-layer} & \multicolumn{2}{c}{56-layer} & \multicolumn{2}{c}{3-layer} & \multicolumn{2}{c}{28-layer} & \multicolumn{2}{c}{56-layer} & \multicolumn{2}{c}{3-layer} & \multicolumn{2}{c}{28-layer} & \multicolumn{2}{c}{56-layer} \\
         \cmidrule(lr){2-3}
         \cmidrule(lr){4-5}
         \cmidrule(lr){6-7}
         \cmidrule(lr){8-9}
         \cmidrule(lr){10-11}
         \cmidrule(lr){12-13}
         \cmidrule(lr){14-15}
         \cmidrule(lr){16-17}
         \cmidrule(lr){18-19}
         & \makecell{SPD} &  \makecell{Acc. (\%)} & \makecell{SPD} &\makecell{Acc. (\%)} & \makecell{SPD} & \makecell{Acc. (\%)} & \makecell{SPD} &  \makecell{Acc. (\%)} & \makecell{SPD} &\makecell{Acc. (\%)} & \makecell{SPD} & \makecell{Acc. (\%)}& \makecell{SPD} &  \makecell{Acc. (\%)} & \makecell{SPD} &\makecell{Acc. (\%)} & \makecell{SPD} & \makecell{Acc. (\%)} \\
         \midrule
         FG & - & 70.72 & - & 70.44 & - & 70.40 & - & 76.01 & - & 75.50 & -  & 74.58 & - & 96.20 & - & 96.13 & - & 96.39  \\
         \thiswork & 1.85$\times$ & 70.57 & 1.90$\times$ & 70.50 & 1.80$\times$ & 70.68 & 1.99$\times$ & 75.44 & 2.33$\times$ & 75.21 & 2.41$\times$ & 74.88 & 2.24$\times$ & 96.06 & 2.37$\times$ & 96.14 & 2.79$\times$ & 96.08  \\
        \bottomrule
    \end{tabular}
    }
    \caption{Speedup and Accuracy of \thiswork}
\end{table*}

==> tables/applications.tex <==
\begin{table}[]
    \centering
    \caption{Benchmark Applications }
    \resizebox{\columnwidth}{!}
    {
    \begin{tabular}{ccccccc}
    \toprule
        \multirowcell{5}{GNN} 
        & \multirowcell{3}{Dataset }
        & Pubmed~\cite{coraciteseerpubmed} & |V| = 2.7K, |E| = 10K\\
        && Citeseer~\cite{coraciteseerpubmed} & |V| = 3.3K , |E| = 3.7K  \\
        && Reddit~\cite{reddit} & |V| = 232M , |E| = 114M  \\
        \cmidrule(lr){2-4}
        &\multirowcell{3}{Environment} & Hidden Dim. & 256 \\
        && HyperCube Dim. & 2 (32\texttimes 32) \\
        %\cmidrule(lr){2-4}
        && Communication & {ReduceScatter \textrightarrow AllReduce} \\
        \midrule
        \multirowcell{5}{DLRM}
        & Dataset &  Criteo~\cite{criteo} & 13 integer, 26 categorical features\\
        \cmidrule(lr){2-4}
        & \multirowcell{3}{Models} &  
          A & Emb dim=16, Tab dim = 128\\
        &&B & Emb dim=16, Tab dim = 64\\
        &&C & Emb dim=64, Tab dim = 128\\
        \cmidrule(lr){2-4}
        & \multirowcell{2}{Environment} & Hypercube Dim. & 1 (1024) \\
        %\cmidrule(lr){2-4}
        && Communication & { AlltoAll  \textrightarrow AlltoAll } \\
        \bottomrule
        
    \end{tabular}
    }
    \label{tab:apps}
\end{table}

==> tables/baselines.tex <==
\begin{table}[]
    \centering
    \small
    \caption{Comparison of \thiswork to Prior Art}
    \label{tab:baselines}
    \resizebox{\columnwidth}{!}
    {
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{cccccccccc}
    \toprule
         \multirowcell{3}{Name}&\multirowcell{3}{Baseline\\Code}&\multicolumn{3}{c}{System} & \multicolumn{3}{c}{Method} \\
         \cmidrule(lr){3-5}
         \cmidrule(lr){6-8}
         & & \makecell{Worker} &  \makecell{Multi-\\server} & \makecell{Multi-\\GPU} &\makecell{Full-\\graph} & \makecell{Mini\\batch} & \makecell{Batch Limit} \\
         \midrule
         PyG~\cite{pyg} & PyG & CPU   & \xmark & N/A & \cmark & \cmark & CPU memory \\
         DGL~\cite{dgl} & DGL & CPU & \xmark & N/A & \cmark & \cmark & CPU memory \\
         AGL~\cite{agl} & Custom & CPU & \cmark & N/A & \cmark & \cmark & CPU memory \\
         
         NeuGraph~\cite{neugraph} & Custom & GPU & \xmark & \cmark & \cmark & \xmark & N/A \\
         NeutronStar~\cite{neutronstar} & LibTorch & GPU & \cmark & \xmark & \cmark & \xmark & N/A \\
         ROC\cite{roc} & FlexFlow & GPU & \cmark & \cmark & \cmark & \xmark & N/A & \\
         PipeGCN~\cite{pipegcn} & DGL & GPU & \cmark & \cmark & \cmark & \xmark & N/A \\
         DistDGL~\cite{distdgl,distdglv2} & DGL & GPU & \cmark & \cmark &  \xmark & \cmark & GPU memory \\
       %  DistDGLv2~\cite{distdglv2} & DGL & GPU & \cmark & \cmark &  \xmark & \cmark & GPU memory \\
         \midrule
         \textbf{\thiswork (Proposed)} & DGL & GPU & \cmark & \cmark & \cmark & \cmark & Aggregate GPUs \\
        \bottomrule
    \end{tabular}
    }%resizebox
\end{table}

==> tables/datasets.tex <==
\begin{table}[]
    \centering
    \resizebox{\columnwidth}{!}
    {
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{ccccccccc}
    \toprule
         \multirowcell{2}{Size}& \multirowcell{2}{Name} &\multicolumn{3}{c}{Dataset Info.} & \multicolumn{3}{c}{Hyper-parameter} \\
         \cmidrule(lr){3-5}
         \cmidrule(lr){6-8}
         & & \makecell{\#Nodes} &  \makecell{\#Edges} & \makecell{Feat. size} &\makecell{lr} & \makecell{Dropout} & \makecell{\#Epochs} \\
         \midrule
         \multirowcell{3}{Small$\sim$\\medium} & ogbn-arxiv~\cite{ogb} & 169K & 1.2M & 128 & 0.01 & 0.5 & 1000 \\
        %\cmidrule(lr){0-7}
          & ogbn-products~\cite{ogb} & 2,449K & 61.9M & 100 & 0.003 & 0.3 & 1000 \\
         & Reddit~\cite{reddit} & 232K & 114.6M & 602 & 0.01 & 0.5 & 1000 \\
         \cmidrule(lr){0-7}
         Hyperscale & ogbn-papers100M~\cite{ogb} & 111M & 1.6B & 128 & 0.01 & 0.5 & 3000 \\
        \bottomrule
    \end{tabular}
    }%resizebox
        \caption{Graph Datasets}
    \label{tab:datasets}
\end{table}

==> tables/environment.tex <==
\begin{table}[]
\footnotesize
\centering
 \def\arraystretch{0.95}
% \resizebox{\columnwidth}{!}
{
\begin{tabular}{cccc}
\toprule
%\multicolumn{3}{c}{\textbf {Common}}\\
\multirowcell{6}[-0.4ex]{\textbf {HW}} 
& \multirowcell{4}{Server} 
& GPU & 4$\times$ NVIDIA RTX A6000 \\
&& CPU & 1$\times$ EPYC 7302, 16C 32T \\
&& Memory & 256GB DDR4 ECC \\
&& Int. connect & NVLink Bridge~\cite{nvbridge} \\
\cmidrule(lr){3-4}
& \multirowcell{2}{Cluster}
& \#Servers & 4 \\
&& Ext. connect & Infiniband QDR (32Gbps) \\


\midrule

\multirowcell{8}[-0.8ex]{\textbf {SW}} 
& \multirow{4}{*}{Common} 
 & Python & 3.10\\
& & PyTorch  & 1.13 \\
& & CUDA & 11.6.2 \\
& & NCCL & 2.10.3 \\

\cmidrule(lr){3-4} 
& \multirow{4}{*}{GNN}
& DGL & 0.9.1~\cite{dgl} \\
&& Model & ResSAGE+~\cite{deepergcn} \\
&& Hidden dim. & 64 \\
&& Task & Node classification \\

 \bottomrule
\end{tabular}
}\caption{Experimental Environment}\label{tab:environment}
\end{table} 

==> tables/oldapplications.tex <==
\begin{table}[]
    \centering
    \caption{Benchmark Applications \JL{info is temporary. plz put your settings!} }
    \resizebox{\columnwidth}{!}
    {
    \begin{tabular}{cccccccc}
    \toprule
        App & Case & type & Hypercube Dim. & Feature width & Collectives \\
        \midrule
        \multirowcell{2}{GNN} 
        & -A & \multirowcell{2}{8b, 16b, 32b} & 2 (32\texttimes 32)& \multirowcell{2}{256}&RS + AR \\ 
        & -B & & 2 (8\texttimes 128)& &AG + AR \\ 
        \midrule
        \multirowcell{}{DLRM} 
        & -TP & \multirowcell{1}{8b} & 1 (1024)& & AA\\ % table par
        %& -3P &  & 3 (16\texttimes 8\texttimes 8)& &AA + AR + AG\\ % 3D par
        \bottomrule
        
    \end{tabular}
    }
    \label{tab:apps}
\end{table}
